Do Crises Increase Parochial Behavior? Evidence from Donations During Covid

Do people behave more favorably towards their in-group during a crisis? Defining in/out-groups by geography, we study donations to local versus non-local charities during the Covid pandemic. The evidence points to increased parochialism: We document a relative increase in donations to local charities and show that donors in high-Covid areas increased their local giving and became less responsive to international disasters. Increased local giving was most pronounced during the first year of the pandemic. Our interpretation is that greater parochialism in donations was due to heightened concern about the immediate impact of Covid at a time when localities were salient.

==> results_figure/main_diff_change_after_covid_totD.tex <==
                    &\multicolumn{7}{c}{Log (Total Donations)}                                                                                                                \\\cmidrule(lr){2-8}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         &\multicolumn{1}{c}{(7)}         \\
\midrule
Post Covid          &      0.1797\sym{***}&                     &      1.5533\sym{***}&      1.5489\sym{***}&      1.5482\sym{***}&      0.0000         &      0.0000         \\
                    &    (0.0171)         &                     &    (0.2269)         &    (0.2250)         &    (0.2251)         &         (.)         &         (.)         \\
\addlinespace
Post Covid $\times$ High Covid&                     &                     &     -0.0724\sym{**} &     -0.0732\sym{**} &     -0.0729\sym{**} &     -0.1215\sym{**} &     -0.0321\sym{***}\\
                    &                     &                     &    (0.0337)         &    (0.0331)         &    (0.0329)         &    (0.0493)         &    (0.0082)         \\
\addlinespace
Post Covid $\times$ Large GDP Shock&                     &                     &                     &      0.0077         &      0.0075         &     -0.0228         &      0.0055         \\
                    &                     &                     &                     &    (0.0354)         &    (0.0357)         &    (0.0393)         &    (0.0096)         \\
\addlinespace
Post Covid $\times$ Strong Local Belonging&                     &                     &                     &                     &      0.0042         &      0.0106         &      0.0067         \\
                    &                     &                     &                     &                     &    (0.0359)         &    (0.0363)         &    (0.0109)         \\
\addlinespace
Year = 2020         &                     &      0.1490\sym{***}&                     &                     &                     &                     &                     \\
                    &                     &    (0.0167)         &                     &                     &                     &                     &                     \\
\addlinespace
Year = 2021         &                     &      0.2409\sym{***}&                     &                     &                     &                     &                     \\
                    &                     &    (0.0206)         &                     &                     &                     &                     &                     \\
\midrule
Obs.                &     423,409         &     423,409         &     410,599         &     410,599         &     410,599         &     410,599         &     243,245         \\
Donor Fixed Effects &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Differential Change by Other Demographic Features&           N         &           N         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Region by Year Fixed Effects&           N         &           N         &           N         &           N         &           N         &           Y         &           Y         \\
Include Only Non-zero Observations&           N         &           N         &           N         &           N         &           N         &           N         &           Y         \\


==> results_table/agg_sep_correlation.tex <==
                    &\multicolumn{3}{c}{Covid Exposure by End of 2022}                \\\cmidrule(lr){2-4}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
High Covid Exposure in 2020&      0.7867\sym{***}&                     &                     \\
                    &    (0.0507)         &                     &                     \\
\addlinespace
High Covid Exposure in 2021&                     &      0.6533\sym{***}&                     \\
                    &                     &    (0.0622)         &                     \\
\addlinespace
High Covid Exposure in 2022&                     &                     &      0.4933\sym{***}\\
                    &                     &                     &    (0.0715)         \\
\addlinespace
Constant            &      0.1067\sym{***}&      0.1733\sym{***}&      0.2533\sym{***}\\
                    &    (0.0359)         &    (0.0440)         &    (0.0506)         \\
\midrule
Obs                 &         150         &         150         &         150         \\
RSquare             &       0.619         &       0.427         &       0.243         \\


==> results_table/befaft_interaction_results.tex <==
                    &\multicolumn{2}{c}{Local Share (by Value)} &\multicolumn{2}{c}{Local Share (by Number)}\\\cmidrule(lr){2-3}\cmidrule(lr){4-5}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\midrule
Post Covid $\times$ Death Rate (in percentage)&      0.2767\sym{**} &      0.1049         &      0.2021\sym{***}&      0.0888         \\
                    &    (0.1080)         &    (0.1351)         &    (0.0625)         &    (0.0701)         \\
\addlinespace
Post Covid $\times$ March-April-May $\times$ Death Rate (in percentage)&                     &      0.5932\sym{***}&                     &      0.3964\sym{***}\\
                    &                     &    (0.2153)         &                     &    (0.1012)         \\
\midrule
Obs.                &      12,600         &      12,600         &      12,600         &      12,600         \\
Mean Outcome        &       0.203         &       0.203         &       0.125         &       0.125         \\
Post Covid          &           Y         &           Y         &           Y         &           Y         \\
Post Covid $\times$ March-April-May&           Y         &           Y         &           Y         &           Y         \\
ULAD Fixed Effects  &           Y         &           Y         &           Y         &           Y         \\
Time Trend          &           Y         &           Y         &           Y         &           Y         \\
Month Fixed Effects &           Y         &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         &           Y         \\
Differential Effects by Socio-demographic Feature&           Y         &           Y         &           Y         &           Y         \\


==> results_table/befaft_local_share.tex <==
                    &\multicolumn{1}{c}{Any Donation}&\multicolumn{2}{c}{Any Local}              &\multicolumn{2}{c}{Local Share (Value)}    &\multicolumn{2}{c}{Local Share (Number)}   \\\cmidrule(lr){2-2}\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}\\
                    &\multicolumn{1}{c}{Full}&\multicolumn{1}{c}{Full}&\multicolumn{1}{c}{Total $>$ 0}&\multicolumn{1}{c}{Full}&\multicolumn{1}{c}{Total $>$ 0}&\multicolumn{1}{c}{Full}&\multicolumn{1}{c}{Total $>$ 0}\\
\midrule
Post Covid          &      0.0222\sym{***}&      0.0039\sym{**} &      0.0071\sym{**} &      0.0022\sym{**} &      0.0042\sym{***}&      0.0019\sym{*}  &      0.0039\sym{**} \\
                    &    (0.0030)         &    (0.0017)         &    (0.0028)         &    (0.0009)         &    (0.0015)         &    (0.0010)         &    (0.0016)         \\
\midrule
Obs                 &     423,423         &     423,423         &     262,648         &     423,423         &     262,648         &     423,423         &     262,648         \\
Mean Outcome        &       0.620         &       0.292         &       0.292         &       0.107         &       0.107         &       0.099         &       0.099         \\
Donor FE            &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Total Donation      &                     &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Sectoral Composition&                     &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\


==> results_table/befaft_on_local_giving.tex <==
                    &\multicolumn{2}{c}{Share of Local Donations}\\\cmidrule(lr){2-3}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         \\
\midrule
Post Covid          &      0.0042\sym{***}&                     \\
                    &    (0.0013)         &                     \\
\addlinespace
Year = 2020         &                     &      0.0093\sym{***}\\
                    &                     &    (0.0014)         \\
\addlinespace
Year = 2021         &                     &     -0.0068\sym{***}\\
                    &                     &    (0.0017)         \\
\midrule
Obs.                &     251,037         &     251,037         \\
Mean Outcome        &       0.167         &       0.167         \\
Share of Zero       &       0.530         &       0.530         \\
Donor Fixed Effects &           Y         &           Y         \\
Year Trend          &           Y         &           Y         \\
Total Donation      &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         \\


==> results_table/befaft_on_local_giving_by_cause.tex <==
                    &\multicolumn{6}{c}{Share of Local Donations}                                                                                       \\\cmidrule(lr){2-7}
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                    &\multicolumn{1}{c}{Social Services}&\multicolumn{1}{c}{Religious}&\multicolumn{1}{c}{Health}&\multicolumn{1}{c}{Edu/Res/Cul}&\multicolumn{1}{c}{Environment}&\multicolumn{1}{c}{Others}\\
\midrule
Post Covid          &      0.0034\sym{**} &     -0.0073\sym{**} &      0.0176\sym{***}&     -0.0085\sym{*}  &      0.0063\sym{**} &      0.0045\sym{*}  \\
                    &    (0.0015)         &    (0.0030)         &    (0.0028)         &    (0.0044)         &    (0.0028)         &    (0.0026)         \\
\midrule
Obs.                &     196,476         &      86,292         &     138,458         &      55,458         &      56,560         &     103,776         \\
Mean Outcome        &       0.074         &       0.344         &       0.179         &       0.251         &       0.141         &       0.110         \\
Share of Zero       &       0.809         &       0.552         &       0.674         &       0.678         &       0.778         &       0.840         \\
Donor Fixed Effects &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\


==> results_table/befaft_on_local_share.tex <==
                    &\multicolumn{1}{c}{Any Local Donation}&\multicolumn{1}{c}{Local Share (Value)}&\multicolumn{1}{c}{Local Share (Count)}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Post Covid          &      0.0072\sym{***}&      0.0042\sym{***}&      0.0038\sym{***}\\
                    &    (0.0025)         &    (0.0013)         &    (0.0014)         \\
\midrule
Obs                 &     251,043         &     251,043         &     251,043         \\
Mean Outcome        &       0.279         &       0.173         &       0.160         \\
Share of Zero       &       0.530         &       0.530         &       0.530         \\
Donor FE            &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         \\


==> results_table/befaft_on_local_share1.tex <==
                    &\multicolumn{1}{c}{Any Local Donation}&\multicolumn{1}{c}{Local Share (Value)}&\multicolumn{1}{c}{Local Share (Count)}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Post Covid          &      0.0072\sym{***}&      0.0042\sym{***}&      0.0038\sym{***}\\
                    &    (0.0025)         &    (0.0013)         &    (0.0014)         \\
\midrule
Obs                 &     251,043         &     251,043         &     251,043         \\
Mean Outcome        &       0.279         &       0.173         &       0.160         \\
Share of Zero       &       0.530         &       0.530         &       0.530         \\
Donor FE            &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         \\


==> results_table/befaft_on_local_share2.tex <==
                    &\multicolumn{1}{c}{Any Local Donation}&\multicolumn{1}{c}{Local Share (Value)}&\multicolumn{1}{c}{Local Share (Count)}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Post Covid          &      0.0062\sym{**} &      0.0038\sym{***}&      0.0036\sym{***}\\
                    &    (0.0025)         &    (0.0013)         &    (0.0014)         \\
\midrule
Obs                 &     284,853         &     284,853         &     284,853         \\
Mean Outcome        &       0.276         &       0.175         &       0.162         \\
Share of Zero       &       0.530         &       0.530         &       0.530         \\
Donor FE            &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         \\


==> results_table/befaft_on_local_share2022.tex <==
                    &\multicolumn{1}{c}{Any Local Donation}&\multicolumn{1}{c}{Local Share (Value)}&\multicolumn{1}{c}{Local Share (Count)}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Post Covid          &      0.0062\sym{**} &      0.0038\sym{***}&      0.0036\sym{***}\\
                    &    (0.0025)         &    (0.0013)         &    (0.0014)         \\
\midrule
Obs                 &     284,853         &     284,853         &     284,853         \\
Mean Outcome        &       0.276         &       0.175         &       0.162         \\
Share of Zero       &       0.530         &       0.530         &       0.530         \\
Donor FE            &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         \\


==> results_table/befaft_on_local_share3.tex <==
                    &\multicolumn{1}{c}{Any Local Donation}&\multicolumn{1}{c}{Local Share (Value)}&\multicolumn{1}{c}{Local Share (Count)}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Post Covid          &      0.0062\sym{**} &      0.0038\sym{***}&      0.0036\sym{***}\\
                    &    (0.0025)         &    (0.0013)         &    (0.0014)         \\
\midrule
Obs                 &     284,853         &     284,853         &     284,853         \\
Mean Outcome        &       0.276         &       0.175         &       0.162         \\
Share of Zero       &       0.530         &       0.530         &       0.530         \\
Donor FE            &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         \\


==> results_table/befaft_on_local_share_by_sector.tex <==
                    &\multicolumn{1}{c}{Social Services}&\multicolumn{1}{c}{Religious}&\multicolumn{1}{c}{Health/MedicalRes}&\multicolumn{1}{c}{Edu/Res/Cul}&\multicolumn{1}{c}{Environment}&\multicolumn{1}{c}{Others/Unclass}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\midrule
Post Covid          &      0.0034\sym{**} &     -0.0073\sym{**} &      0.0176\sym{***}&     -0.0085\sym{*}  &      0.0063\sym{**} &      0.0045\sym{*}  \\
                    &    (0.0015)         &    (0.0030)         &    (0.0028)         &    (0.0044)         &    (0.0028)         &    (0.0026)         \\
\midrule
Obs                 &     196,482         &      86,296         &     138,464         &      55,458         &      56,565         &     103,779         \\
Mean Outcome        &        .074         &        .344         &        .179         &        .252         &        .141         &         .11         \\
Share of Zero       &.8090000000000001         &        .552         &        .674         &        .678         &        .778         &        .839         \\
Donor FE            &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\


==> results_table/befaft_on_local_share_by_year.tex <==
                    &\multicolumn{1}{c}{Any Local Donation}&\multicolumn{1}{c}{Local Share (Value)}&\multicolumn{1}{c}{Local Share (Count)}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Year = 2020         &      0.0155\sym{***}&      0.0093\sym{***}&      0.0080\sym{***}\\
                    &    (0.0026)         &    (0.0014)         &    (0.0014)         \\
\addlinespace
Year = 2021         &     -0.0105\sym{***}&     -0.0068\sym{***}&     -0.0050\sym{***}\\
                    &    (0.0030)         &    (0.0017)         &    (0.0017)         \\
\addlinespace
Year = 2022         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         \\
\midrule
Obs                 &     251,043         &     251,043         &     251,043         \\
Mean Outcome        &       0.279         &       0.173         &       0.160         \\
Share of Zero       &       0.530         &       0.530         &       0.530         \\
Donor FE            &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         \\


==> results_table/befaft_on_local_share_by_year1.tex <==
                    &\multicolumn{1}{c}{Any Local Donation}&\multicolumn{1}{c}{Local Share (Value)}&\multicolumn{1}{c}{Local Share (Count)}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Year = 2020         &      0.0155\sym{***}&      0.0093\sym{***}&      0.0080\sym{***}\\
                    &    (0.0026)         &    (0.0014)         &    (0.0014)         \\
\addlinespace
Year = 2021         &     -0.0105\sym{***}&     -0.0068\sym{***}&     -0.0050\sym{***}\\
                    &    (0.0030)         &    (0.0017)         &    (0.0017)         \\
\addlinespace
Year = 2022         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         \\
\midrule
Obs                 &     251,043         &     251,043         &     251,043         \\
Mean Outcome        &       0.279         &       0.173         &       0.160         \\
Share of Zero       &       0.530         &       0.530         &       0.530         \\
Donor FE            &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         \\


==> results_table/befaft_on_local_share_by_year2.tex <==
                    &\multicolumn{1}{c}{Any Local Donation}&\multicolumn{1}{c}{Local Share (Value)}&\multicolumn{1}{c}{Local Share (Count)}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Year = 2020         &      0.0147\sym{***}&      0.0090\sym{***}&      0.0077\sym{***}\\
                    &    (0.0027)         &    (0.0014)         &    (0.0014)         \\
\addlinespace
Year = 2021         &     -0.0115\sym{***}&     -0.0070\sym{***}&     -0.0051\sym{***}\\
                    &    (0.0030)         &    (0.0016)         &    (0.0017)         \\
\addlinespace
Year = 2022         &      0.0049         &      0.0058         &      0.0054         \\
                    &    (0.0062)         &    (0.0041)         &    (0.0035)         \\
\midrule
Obs                 &     284,853         &     284,853         &     284,853         \\
Mean Outcome        &       0.276         &       0.175         &       0.162         \\
Share of Zero       &       0.530         &       0.530         &       0.530         \\
Donor FE            &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         \\


==> results_table/befaft_on_local_share_by_year2022.tex <==
                    &\multicolumn{1}{c}{Any Local Donation}&\multicolumn{1}{c}{Local Share (Value)}&\multicolumn{1}{c}{Local Share (Count)}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Year = 2020         &      0.0155\sym{***}&      0.0093\sym{***}&      0.0080\sym{***}\\
                    &    (0.0026)         &    (0.0014)         &    (0.0014)         \\
\addlinespace
Year = 2021         &     -0.0105\sym{***}&     -0.0068\sym{***}&     -0.0050\sym{***}\\
                    &    (0.0030)         &    (0.0017)         &    (0.0017)         \\
\addlinespace
Year = 2022         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         \\
\midrule
Obs                 &     251,043         &     251,043         &     251,043         \\
Mean Outcome        &       0.279         &       0.173         &       0.160         \\
Share of Zero       &       0.530         &       0.530         &       0.530         \\
Donor FE            &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         \\


==> results_table/befaft_on_local_share_by_year3.tex <==
                    &\multicolumn{1}{c}{Any Local Donation}&\multicolumn{1}{c}{Local Share (Value)}&\multicolumn{1}{c}{Local Share (Count)}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Year = 2020         &      0.0147\sym{***}&      0.0090\sym{***}&      0.0077\sym{***}\\
                    &    (0.0027)         &    (0.0014)         &    (0.0014)         \\
\addlinespace
Year = 2021         &     -0.0115\sym{***}&     -0.0070\sym{***}&     -0.0051\sym{***}\\
                    &    (0.0030)         &    (0.0016)         &    (0.0017)         \\
\addlinespace
Year = 2022         &      0.0049         &      0.0058         &      0.0054         \\
                    &    (0.0062)         &    (0.0041)         &    (0.0035)         \\
\midrule
Obs                 &     284,853         &     284,853         &     284,853         \\
Mean Outcome        &       0.276         &       0.175         &       0.162         \\
Share of Zero       &       0.530         &       0.530         &       0.530         \\
Donor FE            &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         \\


==> results_table/befaft_on_overseas_share.tex <==
                    &\multicolumn{2}{c}{Overseas Share (Value)} &\multicolumn{2}{c}{Overseas Share (Number)}&\multicolumn{2}{c}{}                       &\multicolumn{2}{c}{}                       \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\
                    &\multicolumn{1}{c}{Full}&\multicolumn{1}{c}{Total $>$ 0}&\multicolumn{1}{c}{Full}&\multicolumn{1}{c}{Total $>$ 0}&\multicolumn{1}{c}{Full}&\multicolumn{1}{c}{Total $>$ 0}&\multicolumn{1}{c}{est7}&\multicolumn{1}{c}{est8}\\
\midrule
Post Covid          &      0.0038\sym{***}&      0.0070\sym{***}&      0.0017\sym{*}  &      0.0035\sym{**} &      0.0019\sym{***}&      0.0034\sym{***}&      0.0009         &      0.0016\sym{*}  \\
                    &    (0.0011)         &    (0.0018)         &    (0.0010)         &    (0.0018)         &    (0.0006)         &    (0.0009)         &    (0.0006)         &    (0.0009)         \\
\midrule
Obs                 &     423,423         &     262,648         &     423,423         &     262,648         &     423,423         &     262,648         &     423,423         &     262,648         \\
Mean Outcome        &       0.273         &       0.273         &       0.280         &       0.280         &       0.079         &       0.079         &       0.079         &       0.079         \\
Donor FE            &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\


==> results_table/befaft_on_sectoral_giving.tex <==
                    &\multicolumn{6}{c}{Donation Share by Sector}                                                                                       \\\cmidrule(lr){2-7}
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                    &\multicolumn{1}{c}{Social Services}&\multicolumn{1}{c}{Religious}&\multicolumn{1}{c}{Health}&\multicolumn{1}{c}{Edu/Res/Cul}&\multicolumn{1}{c}{Environment}&\multicolumn{1}{c}{Others}\\
\midrule
Post Covid          &      0.0116\sym{***}&     -0.0039\sym{***}&     -0.0114\sym{***}&      0.0019         &      0.0004         &      0.0013         \\
                    &    (0.0017)         &    (0.0011)         &    (0.0018)         &    (0.0012)         &    (0.0007)         &    (0.0012)         \\
\midrule
Obs.                &     251,037         &     251,037         &     251,037         &     251,037         &     251,037         &     251,037         \\
Mean Outcome        &       0.427         &       0.157         &       0.189         &       0.062         &       0.060         &       0.105         \\
Share of Zero       &       0.212         &       0.642         &       0.432         &       0.753         &       0.752         &       0.563         \\
Donor Fixed Effects &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\


==> results_table/befaft_on_sectoral_share.tex <==
                    &\multicolumn{1}{c}{Social Services}&\multicolumn{1}{c}{Religious}&\multicolumn{1}{c}{Health/MedicalRes}&\multicolumn{1}{c}{Edu/Res/Cul}&\multicolumn{1}{c}{Environment}&\multicolumn{1}{c}{Others/Unclass}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\midrule
Post Covid          &      0.0116\sym{***}&     -0.0040\sym{***}&     -0.0114\sym{***}&      0.0019         &      0.0004         &      0.0013         \\
                    &    (0.0017)         &    (0.0011)         &    (0.0018)         &    (0.0012)         &    (0.0007)         &    (0.0012)         \\
\midrule
Obs                 &     251,043         &     251,043         &     251,043         &     251,043         &     251,043         &     251,043         \\
Mean Outcome        &       0.427         &       0.158         &       0.189         &       0.062         &       0.060         &       0.105         \\
Share of Zero       &       0.212         &       0.642         &       0.432         &       0.753         &       0.752         &       0.563         \\
Donor FE            &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\


==> results_table/befaft_on_share_by_geo.tex <==
                    &\multicolumn{1}{c}{Local Share}&\multicolumn{1}{c}{National Share}&\multicolumn{1}{c}{Nat/Overseas Share}&\multicolumn{1}{c}{Overseas Share}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\midrule
Post Covid          &      0.0042\sym{***}&     -0.0132\sym{***}&      0.0056\sym{***}&      0.0034\sym{***}\\
                    &    (0.0013)         &    (0.0017)         &    (0.0012)         &    (0.0008)         \\
\midrule
Obs                 &     251,043         &     251,043         &     251,043         &     251,043         \\
Mean Outcome        &       0.173         &       0.482         &       0.218         &       0.127         \\
Share of Zero       &       0.530         &       0.157         &       0.370         &       0.555         \\
Donor FE            &           Y         &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         &           Y         \\


==> results_table/befaft_on_share_by_geo_congive.tex <==
                    &\multicolumn{2}{c}{Local Share}            &\multicolumn{2}{c}{National Share}         &\multicolumn{2}{c}{Nat/Overseas Share}     &\multicolumn{2}{c}{Overseas Share}         \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\
                    &\multicolumn{1}{c}{Value}&\multicolumn{1}{c}{Count}&\multicolumn{1}{c}{Value}&\multicolumn{1}{c}{Count}&\multicolumn{1}{c}{Value}&\multicolumn{1}{c}{Count}&\multicolumn{1}{c}{Value}&\multicolumn{1}{c}{Count}\\
\midrule
Post Covid          &      0.0042\sym{***}&      0.0039\sym{**} &     -0.0112\sym{***}&     -0.0073\sym{***}&      0.0036\sym{**} &      0.0019         &      0.0034\sym{***}&      0.0016\sym{*}  \\
                    &    (0.0015)         &    (0.0016)         &    (0.0020)         &    (0.0020)         &    (0.0016)         &    (0.0016)         &    (0.0009)         &    (0.0009)         \\
\midrule
Obs                 &     262,648         &     262,648         &     262,648         &     262,648         &     262,648         &     262,648         &     262,648         &     262,648         \\
Mean Outcome        &       0.107         &       0.099         &       0.240         &       0.241         &       0.195         &       0.200         &       0.079         &       0.079         \\
Donor FE            &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\


==> results_table/charity_befaft_local_donor.tex <==
                    &\multicolumn{2}{c}{Log Donation Value}     &\multicolumn{2}{c}{Log Donation Count}     \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}
                    &\multicolumn{1}{c}{Donation $>$ 0}&\multicolumn{1}{c}{Count = 7}&\multicolumn{1}{c}{Donation $>$ 0}&\multicolumn{1}{c}{Count = 7}\\
& (1) & (2) & (3) & (4) \\ \midrule
from Local Donor $\times$ Post&      0.2759\sym{***}&      0.2818\sym{***}&      0.2539\sym{***}&      0.2220\sym{***}\\
                    &    (0.0180)         &    (0.0207)         &    (0.0156)         &    (0.0170)         \\
\addlinespace
from NonLocal Donor $\times$ Post&     -0.3528\sym{***}&     -0.5745\sym{***}&     -0.3226\sym{***}&     -0.5467\sym{***}\\
                    &    (0.0432)         &    (0.0506)         &    (0.0333)         &    (0.0479)         \\
\midrule
Obs                 &      94,838         &      39,349         &      94,838         &      39,349         \\
Charity FE          &           Y         &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         \\


==> results_table/charity_commission_evidence.tex <==
& \multicolumn{6}{c}{Log Total Donation} \\\cmidrule(lr){2-7}
                                        & \multicolumn{1}{c}{(1)} & \multicolumn{1}{c}{(2)} & \multicolumn{1}{c}{(3)} & \multicolumn{1}{c}{(4)} & \multicolumn{1}{c}{(5)} & \multicolumn{1}{c}{(6)} \\
\midrule
Post Covid                              & 0.159\sym{***}          & 0.170\sym{***}          &                         &                         &                         &                         \\
                                        & (0.025)                 & (0.025)                 &                         &                         &                         &                         \\
\addlinespace
Post Covid $\times$ Local               & 0.086\sym{***}          & 0.090\sym{***}          &                         &                         &                         &                         \\
                                        & (0.027)                 & (0.027)                 &                         &                         &                         &                         \\
\addlinespace
Year = 2020                             &                         &                         & 0.205\sym{***}          & 0.181\sym{***}          & 0.171\sym{***}          & 0.187\sym{***}          \\
                                        &                         &                         & (0.027)                 & (0.027)                 & (0.030)                 & (0.041)                 \\
\addlinespace
Year = 2020 $\times$ Local              &                         &                         & 0.202\sym{***}          & 0.209\sym{***}          & 0.226\sym{***}          & 0.216\sym{***}          \\
                                        &                         &                         & (0.033)                 & (0.033)                 & (0.040)                 & (0.041)                 \\
\addlinespace
Year = 2021                             &                         &                         & 0.124\sym{***}          & 0.118\sym{***}          & 0.107\sym{***}          & 0.101\sym{**}           \\
                                        &                         &                         & (0.029)                 & (0.028)                 & (0.032)                 & (0.040)                 \\
\addlinespace
Year = 2021 $\times$ Local              &                         &                         & 0.011                   & 0.014                   & 0.034                   & 0.047                   \\
                                        &                         &                         & (0.031)                 & (0.030)                 & (0.043)                 & (0.037)                 \\
\addlinespace
(log) Fundraising Spending              &                         & 0.005\sym{***}          & 0.004\sym{***}          & 0.005\sym{***}          & 0.005\sym{***}          & 0.004\sym{*}            \\
                                        &                         & (0.002)                 & (0.002)                 & (0.002)                 & (0.002)                 & (0.002)                 \\
\midrule
Observations                            & 68,873                  & 68,856                  & 68,856                  & 64,924                  & 64,924                  & 48,706                  \\
R-squared                               & 0.83                    & 0.83                    & 0.83                    & 0.84                    & 0.84                    & 0.83                    \\
Charity Fixed Effects                   & Y                       & Y                       & Y                       & Y                       & Y                       & Y                       \\
Time Trend                              & Y                       & Y                       & Y                       & Y                       & N                       & Y                       \\
Time Trend for Local/Nonlocal Charities & N                       & N                       & N                       & N                       & Y                       & N                       \\
Log GDP Per Capita                      & N                       & N                       & N                       & Y                       & Y                       & Y                       \\
London Charities Included               & Y                       & Y                       & Y                       & Y                       & Y                       & N                       \\

==> results_table/charity_commission_imputed.tex <==
& \multicolumn{3}{c}{Log Total Donation} \\ \cmidrule(lr){2-4}
                    & \multicolumn{1}{c}{(1)} & \multicolumn{1}{c}{(2)} & \multicolumn{1}{c}{(3)} \\
\midrule
Post Covid          & 0.130\sym{***}          &                         &                         \\
                    & (0.026)                 &                         &                         \\
\addlinespace
Post Covid $\times$ Local & 0.100\sym{***}       &                         &                         \\
                    & (0.026)                 &                         &                         \\
\addlinespace
Year = 2020                 &                         & 0.128\sym{***}          & 0.131\sym{***}          \\
                    &                         & (0.025)                 & (0.025)                 \\
\addlinespace
Year = 2020 $\times$ Local  &                         & 0.175\sym{***}          & 0.169\sym{***}          \\
                    &                         & (0.030)                 & (0.033)                 \\
\addlinespace
Year = 2021                 &                         & 0.123\sym{***}          & 0.127\sym{***}          \\
                    &                         & (0.029)                 & (0.029)                 \\
\addlinespace
Year = 2021 $\times$ Local  &                         & 0.045                   & 0.039                   \\
                    &                         & (0.028)                 & (0.035)                 \\
\midrule
Observations        & 94,973                  & 94,973                   & 94,973                    \\
R-squared           & 0.84                    & 0.84                    & 0.84                    \\
charity FE          & Yes                     & Yes                     & Yes                     \\
Time Trend          & Yes                     & Yes                     & Yes                     \\
Time Trend for Local/Nonlocal Charities & No  & No                      & Yes                     \\

==> results_table/charity_covid_health_local_donor.tex <==
                    &\multicolumn{4}{c}{Log Donation Value}                                                 \\\cmidrule(lr){2-5}
                    &\multicolumn{1}{c}{Donation $>$ 0}&\multicolumn{1}{c}{Donation $>$ 0}&\multicolumn{1}{c}{Count = 7}&\multicolumn{1}{c}{Count = 7}\\
& (1) & (2) & (3) & (4) \\ \midrule
from Local Donor $\times$ Post $\times$ High Covid $\times$ Health&      0.4169\sym{***}&      0.1932\sym{***}&      0.5083\sym{***}&      0.1354         \\
                    &    (0.0583)         &    (0.0584)         &    (0.0930)         &    (0.0886)         \\
\addlinespace
from Local Donor $\times$ Post $\times$ High Covid $\times$ NonHealth&      0.2351\sym{***}&      0.0948\sym{***}&      0.2685\sym{***}&      0.0534\sym{*}  \\
                    &    (0.0251)         &    (0.0269)         &    (0.0309)         &    (0.0311)         \\
\addlinespace
from Local Donor $\times$ Post $\times$ Low Covid $\times$ Health&      0.4167\sym{***}&      0.1945\sym{***}&      0.4407\sym{***}&      0.0866\sym{*}  \\
                    &    (0.0425)         &    (0.0407)         &    (0.0484)         &    (0.0496)         \\
\addlinespace
from Local Donor $\times$ Post $\times$ Low Covid $\times$ NonHealth&      0.2719\sym{***}&      0.1244\sym{***}&      0.2468\sym{***}&      0.0153         \\
                    &    (0.0244)         &    (0.0234)         &    (0.0285)         &    (0.0264)         \\
\addlinespace
from NonLocal Donor $\times$ Post $\times$ High Covid $\times$ Health&     -0.5375\sym{***}&     -0.0903         &     -0.8163\sym{***}&     -0.2211\sym{*}  \\
                    &    (0.1234)         &    (0.1168)         &    (0.1183)         &    (0.1159)         \\
\addlinespace
from NonLocal Donor $\times$ Post $\times$ High Covid $\times$ NonHealth&     -0.2793\sym{***}&      0.1441\sym{***}&     -0.5020\sym{***}&      0.0489         \\
                    &    (0.0599)         &    (0.0497)         &    (0.0749)         &    (0.0627)         \\
\addlinespace
from NonLocal Donor $\times$ Post $\times$ Low Covid $\times$ Health&     -0.6171\sym{***}&     -0.1573\sym{*}  &     -0.8407\sym{***}&     -0.2384\sym{***}\\
                    &    (0.0819)         &    (0.0818)         &    (0.0768)         &    (0.0879)         \\
\addlinespace
from NonLocal Donor $\times$ Post $\times$ Low Covid $\times$ NonHealth&     -0.3293\sym{***}&      0.1165\sym{***}&     -0.5254\sym{***}&      0.0556         \\
                    &    (0.0577)         &    (0.0377)         &    (0.0712)         &    (0.0408)         \\
\midrule
Obs                 &      94,838         &      94,838         &      39,349         &      39,349         \\
Charity FE          &           Y         &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         \\
Year Trend By Donor Type&                     &           Y         &                     &           Y         \\


==> results_table/charity_covid_local_donor.tex <==
                    &\multicolumn{4}{c}{Log Donation Value}                                                 \\\cmidrule(lr){2-5}
                    &\multicolumn{1}{c}{Donation $>$ 0}&\multicolumn{1}{c}{Donation $>$ 0}&\multicolumn{1}{c}{Count = 7}&\multicolumn{1}{c}{Count = 7}\\
& (1) & (2) & (3) & (4) \\ \midrule
from Local Donor $\times$ Post $\times$ High Covid&      0.2568\sym{***}&      0.1063\sym{***}&      0.3019\sym{***}&      0.0647\sym{**} \\
                    &    (0.0230)         &    (0.0256)         &    (0.0270)         &    (0.0297)         \\
\addlinespace
from Local Donor $\times$ Post $\times$ Low  Covid&      0.2876\sym{***}&      0.1318\sym{***}&      0.2703\sym{***}&      0.0236         \\
                    &    (0.0241)         &    (0.0226)         &    (0.0268)         &    (0.0243)         \\
\addlinespace
from NonLocal Donor $\times$ Post $\times$ High Covid&     -0.3215\sym{***}&      0.1076\sym{**} &     -0.5654\sym{***}&     -0.0025         \\
                    &    (0.0603)         &    (0.0502)         &    (0.0710)         &    (0.0613)         \\
\addlinespace
from NonLocal Donor $\times$ Post $\times$ Low  Covid&     -0.3721\sym{***}&      0.0776\sym{**} &     -0.5797\sym{***}&      0.0074         \\
                    &    (0.0559)         &    (0.0371)         &    (0.0651)         &    (0.0377)         \\
\midrule
Obs                 &      94,838         &      94,838         &      39,349         &      39,349         \\
Charity FE          &           Y         &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         \\
Year Trend By Donor Type&                     &           Y         &                     &           Y         \\


==> results_table/charity_media_local_donor.tex <==
                    &\multicolumn{2}{c}{Log Donation Value}     \\\cmidrule(lr){2-3}
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}\\
                    &\multicolumn{1}{c}{Donation $>$ 0}&\multicolumn{1}{c}{Count = 7}\\
\midrule
from Local Donor $\times$ Post $\times$ High Covid $\times$ High Media&      0.2584\sym{***}&      0.3731\sym{***}\\
                    &    (0.0216)         &    (0.0245)         \\
\addlinespace
from Local Donor $\times$ Post $\times$ Low Covid $\times$ High Media&      0.2653\sym{***}&      0.3013\sym{***}\\
                    &    (0.0265)         &    (0.0336)         \\
\addlinespace
from NonLocal Donor $\times$ Post $\times$ High Covid $\times$ High Media&     -0.3485\sym{***}&     -0.5160\sym{***}\\
                    &    (0.0711)         &    (0.0782)         \\
\addlinespace
from NonLocal Donor $\times$ Post $\times$ Low Covid $\times$ High Media&     -0.3536\sym{***}&     -0.4905\sym{***}\\
                    &    (0.0723)         &    (0.0807)         \\
\addlinespace
from Local Donor $\times$ Post $\times$ High Covid $\times$ Low Media&      0.2514\sym{***}&      0.3193\sym{***}\\
                    &    (0.0646)         &    (0.0757)         \\
\addlinespace
from Local Donor $\times$ Post $\times$ Low Covid $\times$ Low Media&      0.3415\sym{***}&      0.4053\sym{***}\\
                    &    (0.0385)         &    (0.0376)         \\
\addlinespace
from NonLocal Donor $\times$ Post $\times$ High Covid $\times$ High Media&     -0.2388\sym{***}&     -0.4682\sym{***}\\
                    &    (0.0913)         &    (0.1360)         \\
\addlinespace
from NonLocal Donor $\times$ Post $\times$ Low Covid $\times$ Low Media&     -0.4197\sym{***}&     -0.5949\sym{***}\\
                    &    (0.0567)         &    (0.0606)         \\
\midrule
Obs                 &      94,838         &      39,349         \\
Charity FE          &           Y         &           Y         \\
Year Trend          &           Y         &           Y         \\
Year Trend By Donor Type&                     &                     \\


==> results_table/community_on_local_giving.tex <==
\\ \multicolumn{2}{l}{\textbf{Panel A:}} \\
                    &\multicolumn{1}{c}{Any Local Donation}&\multicolumn{1}{c}{Local Share (Value)}&\multicolumn{1}{c}{Local Share (Count)}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Low Local Belonging $\times$ Post&     -0.0036         &     -0.0022         &     -0.0011         \\
                    &    (0.0053)         &    (0.0022)         &    (0.0022)         \\
\addlinespace
High Local Belonging $\times$ Post&      0.0127\sym{***}&      0.0074\sym{***}&      0.0064\sym{***}\\
                    &    (0.0026)         &    (0.0015)         &    (0.0015)         \\
\midrule \\ \multicolumn{2}{l}{\textbf{Panel B:}} \\
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Low Hate-crime $\times$ Post&      0.0208\sym{***}&      0.0096\sym{***}&      0.0081\sym{***}\\
                    &    (0.0032)         &    (0.0017)         &    (0.0017)         \\
\addlinespace
High Hate-crime $\times$ Post&     -0.0106\sym{**} &     -0.0029         &     -0.0018         \\
                    &    (0.0047)         &    (0.0019)         &    (0.0018)         \\
\midrule \\ \multicolumn{2}{l}{\textbf{Panel C:}} \\
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Low Ethnic Homogeneity $\times$ Post&     -0.0051         &     -0.0013         &     -0.0006         \\
                    &    (0.0049)         &    (0.0023)         &    (0.0022)         \\
\addlinespace
High Ethnic Homogeneity $\times$ Post&      0.0191\sym{***}&      0.0094\sym{***}&      0.0082\sym{***}\\
                    &    (0.0038)         &    (0.0018)         &    (0.0017)         \\
\midrule
Obs.                &     251,037         &     251,037         &     251,037         \\
Mean outcome        &       0.470         &       0.173         &       0.160         \\
Donor FE            &           Y         &           Y         &           Y         \\
Year trend          &           Y         &           Y         &           Y         \\
Total donation control&           Y         &           Y         &           Y         \\
Sectoral composition controls&           Y         &           Y         &           Y         \\


==> results_table/covariants_with_local_giving.tex <==
            &\multicolumn{3}{c}{Share of Local Donations}                     \\\cmidrule(lr){2-4}
            &LPM (All Donors)         &LPM (DonCount $\ge$ 5)         &       Tobit         \\
\midrule
main        &                     &                     &                     \\
Male        &      0.0062\sym{**} &      0.0046         &      0.0062\sym{**} \\
            &    (0.0027)         &    (0.0032)         &    (0.0027)         \\
\addlinespace
Wealth Index&      0.0003\sym{***}&      0.0004\sym{***}&      0.0003\sym{***}\\
            &    (0.0001)         &    (0.0001)         &    (0.0001)         \\
\addlinespace
Urban       &      0.0134\sym{***}&      0.0144\sym{***}&      0.0134\sym{***}\\
            &    (0.0036)         &    (0.0041)         &    (0.0036)         \\
\addlinespace
Higher Education&      1.5641         &      3.5337\sym{**} &      1.5641         \\
            &    (1.5947)         &    (1.7328)         &    (1.5946)         \\
\addlinespace
Age 65+     &     -4.3063\sym{**} &     -3.5326\sym{**} &     -4.3063\sym{**} \\
            &    (1.8390)         &    (1.6600)         &    (1.8389)         \\
\addlinespace
British White&     -0.5123         &     -1.2177         &     -0.5123         \\
            &    (2.0587)         &    (2.2432)         &    (2.0585)         \\
\addlinespace
Religious   &     -2.9328         &     -4.1155\sym{**} &     -2.9328         \\
            &    (1.9181)         &    (2.0012)         &    (1.9180)         \\
\addlinespace
Self-claim UK Identity&      9.4776\sym{***}&      9.8514\sym{***}&      9.4776\sym{***}\\
            &    (2.7709)         &    (3.1850)         &    (2.7707)         \\
\addlinespace
Conservative Vote Share&     -0.0208         &      0.0094         &     -0.0208         \\
            &    (0.0434)         &    (0.0490)         &    (0.0434)         \\
\addlinespace
Labour Vote Share&      0.0564         &      0.0788\sym{*}  &      0.0564         \\
            &    (0.0432)         &    (0.0471)         &    (0.0432)         \\
\addlinespace
LibDem Vote Share&      0.0718\sym{*}  &      0.0907\sym{**} &      0.0718\sym{*}  \\
            &    (0.0392)         &    (0.0422)         &    (0.0392)         \\
\addlinespace
High Hate-Crime Area&     -0.0044         &     -0.0056         &     -0.0044         \\
            &    (0.0051)         &    (0.0056)         &    (0.0051)         \\
\addlinespace
Ethnic Homogeneity&      0.1587\sym{***}&      0.1617\sym{***}&      0.1587\sym{***}\\
            &    (0.0470)         &    (0.0472)         &    (0.0470)         \\
\addlinespace
Sense of Local Belonging&     -0.0102         &     -0.0194         &     -0.0102         \\
            &    (0.0169)         &    (0.0194)         &    (0.0169)         \\
\addlinespace
High Covid Exposure&     -0.0015         &     -0.0012         &     -0.0015         \\
            &    (0.0045)         &    (0.0045)         &    (0.0045)         \\
\midrule
Obs.        &     175,091         &     112,180         &     175,091         \\
Sectoral Composition&           Y         &           Y         &           Y         \\
Year Fixed Effects&           Y         &           Y         &           Y         \\


==> results_table/covariation_with_local_giving.tex <==
            &\multicolumn{3}{c}{Any Local Donation}                           &\multicolumn{3}{c}{Local Share (Value)}                          \\\cmidrule(lr){2-4}\cmidrule(lr){5-7}
            &   LPM (All)         &LPM (Don Count ≥ 5)         &       Tobit         &   LPM (All)         &LPM (Don Count ≥ 5)         &       Tobit         \\
\midrule
main        &                     &                     &                     &                     &                     &                     \\
Male        &      -0.004         &       0.003         &      -0.004         &       0.006\sym{**} &       0.005         &       0.006\sym{**} \\
            &     (0.005)         &     (0.007)         &     (0.005)         &     (0.003)         &     (0.003)         &     (0.003)         \\
\addlinespace
Wealth Index&       0.000\sym{**} &       0.001\sym{***}&       0.000\sym{**} &       0.000\sym{***}&       0.000\sym{***}&       0.000\sym{***}\\
            &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         \\
\addlinespace
Urban       &       0.029\sym{***}&       0.034\sym{***}&       0.029\sym{***}&       0.014\sym{***}&       0.015\sym{***}&       0.014\sym{***}\\
            &     (0.006)         &     (0.008)         &     (0.006)         &     (0.003)         &     (0.004)         &     (0.003)         \\
\addlinespace
Level-4 Qual. (\%)&       0.001\sym{*}  &       0.001\sym{***}&       0.001\sym{*}  &       0.000         &       0.000\sym{*}  &       0.000         \\
            &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         \\
\addlinespace
Age 65+ (\%)&       0.000         &       0.000         &       0.000         &      -0.000\sym{**} &      -0.000\sym{**} &      -0.000\sym{**} \\
            &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         \\
\addlinespace
British White (\%)&      -0.000         &      -0.000         &      -0.000         &      -0.000         &      -0.000         &      -0.000         \\
            &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         \\
\addlinespace
Religious (\%)&       0.000         &       0.000         &       0.000         &      -0.000         &      -0.000\sym{**} &      -0.000         \\
            &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         \\
\addlinespace
Self-claim UK Identity (\%)&       0.002\sym{***}&       0.002\sym{***}&       0.002\sym{***}&       0.001\sym{***}&       0.001\sym{***}&       0.001\sym{***}\\
            &     (0.000)         &     (0.001)         &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         \\
\addlinespace
Conservative Vote Share&       0.100         &       0.130         &       0.100         &      -0.021         &       0.009         &      -0.021         \\
            &     (0.083)         &     (0.109)         &     (0.083)         &     (0.042)         &     (0.047)         &     (0.042)         \\
\addlinespace
Labour Vote Share&       0.139\sym{*}  &       0.146         &       0.139\sym{*}  &       0.057         &       0.080\sym{*}  &       0.057         \\
            &     (0.083)         &     (0.108)         &     (0.083)         &     (0.042)         &     (0.045)         &     (0.042)         \\
\addlinespace
LibDem Vote Share&       0.168\sym{**} &       0.191\sym{*}  &       0.168\sym{**} &       0.072\sym{*}  &       0.090\sym{**} &       0.072\sym{*}  \\
            &     (0.076)         &     (0.098)         &     (0.076)         &     (0.038)         &     (0.040)         &     (0.038)         \\
\addlinespace
High Hate-Crime Area&      -0.013         &      -0.017         &      -0.013         &      -0.004         &      -0.005         &      -0.004         \\
            &     (0.009)         &     (0.011)         &     (0.009)         &     (0.005)         &     (0.005)         &     (0.005)         \\
\addlinespace
Ethnic Homogeneity&       0.142\sym{*}  &       0.084         &       0.142\sym{*}  &       0.157\sym{***}&       0.162\sym{***}&       0.157\sym{***}\\
            &     (0.079)         &     (0.087)         &     (0.079)         &     (0.047)         &     (0.046)         &     (0.047)         \\
\midrule
Obs         &     175,091         &     112,180         &     175,091         &     175,091         &     112,180         &     175,091         \\
Sectoral Composition&           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Year FEs    &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\


==> results_table/covid_media_on_local_share.tex <==
                    &\multicolumn{2}{c}{Any Local}              &\multicolumn{2}{c}{Local Share (Value)}    &\multicolumn{2}{c}{Local Share (Number)}   \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
                    &\multicolumn{1}{c}{Full}&\multicolumn{1}{c}{Total $>$ 0}&\multicolumn{1}{c}{Full}&\multicolumn{1}{c}{Total $>$ 0}&\multicolumn{1}{c}{Full}&\multicolumn{1}{c}{Total $>$ 0}\\
& (1) & (2) & (3) & (4) &(5) & (6) \\ \midrule
High Covid $\times$ Post&      0.0039         &      0.0050         &      0.0015         &      0.0051         &      0.0013         &      0.0050         \\
                    &    (0.0055)         &    (0.0083)         &    (0.0031)         &    (0.0041)         &    (0.0028)         &    (0.0036)         \\
\addlinespace
Low Covid $\times$ Post&     -0.0045         &     -0.0077         &     -0.0028         &     -0.0025         &     -0.0023         &     -0.0008         \\
                    &    (0.0041)         &    (0.0064)         &    (0.0019)         &    (0.0026)         &    (0.0019)         &    (0.0025)         \\
\addlinespace
High Media $\times$ Post&      0.0079\sym{*}  &      0.0146\sym{*}  &      0.0049\sym{**} &      0.0056\sym{*}  &      0.0042\sym{*}  &      0.0037         \\
                    &    (0.0047)         &    (0.0075)         &    (0.0024)         &    (0.0033)         &    (0.0023)         &    (0.0030)         \\
\addlinespace
Low Media $\times$ Post&      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
\midrule
Obs                 &     423,423         &     262,648         &     423,423         &     262,648         &     423,423         &     262,648         \\
Mean Outcome        &       0.292         &       0.470         &       0.107         &       0.173         &       0.099         &       0.160         \\
Donor FE            &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\


==> results_table/covid_media_on_local_share2.tex <==
                    &\multicolumn{2}{c}{Any Local}              &\multicolumn{2}{c}{Local Share (Value)}    &\multicolumn{2}{c}{Local Share (Number)}   \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
                    &\multicolumn{1}{c}{Full}&\multicolumn{1}{c}{Total $>$ 0}&\multicolumn{1}{c}{Full}&\multicolumn{1}{c}{Total $>$ 0}&\multicolumn{1}{c}{Full}&\multicolumn{1}{c}{Total $>$ 0}\\
& (1) & (2) & (3) & (4) &(5) & (6) \\ \midrule
High Covid $\times$ Post&      0.0084\sym{*}  &      0.0127\sym{*}  &      0.0043\sym{*}  &      0.0076\sym{**} &      0.0037\sym{*}  &      0.0058\sym{**} \\
                    &    (0.0050)         &    (0.0072)         &    (0.0024)         &    (0.0030)         &    (0.0021)         &    (0.0027)         \\
\addlinespace
High Media $\times$ Post&      0.0079\sym{*}  &      0.0146\sym{*}  &      0.0049\sym{**} &      0.0056\sym{*}  &      0.0042\sym{*}  &      0.0037         \\
                    &    (0.0047)         &    (0.0075)         &    (0.0024)         &    (0.0033)         &    (0.0023)         &    (0.0030)         \\
\midrule
Obs                 &     423,423         &     262,648         &     423,423         &     262,648         &     423,423         &     262,648         \\
Mean Outcome        &       0.292         &       0.470         &       0.107         &       0.173         &       0.099         &       0.160         \\
Donor FE            &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Postcovid           &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\


==> results_table/covid_on_geo_composition_value.tex <==
                    &\multicolumn{1}{c}{Local Share}&\multicolumn{1}{c}{National Share}&\multicolumn{1}{c}{Nat/Overseas Share}&\multicolumn{1}{c}{Overseas Share}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\midrule
High Covid $\times$ Post&      0.0096\sym{***}&     -0.0212\sym{***}&      0.0083\sym{***}&      0.0033\sym{***}\\
                    &    (0.0022)         &    (0.0022)         &    (0.0014)         &    (0.0011)         \\
\addlinespace
Low Covid $\times$ Post&      0.0013         &     -0.0090\sym{***}&      0.0042\sym{***}&      0.0035\sym{***}\\
                    &    (0.0015)         &    (0.0020)         &    (0.0013)         &    (0.0010)         \\
\midrule
Obs                 &     251,043         &     251,043         &     251,043         &     251,043         \\
Mean Outcome        &       0.173         &       0.482         &       0.218         &       0.127         \\
P(diff)             &       0.002         &       0.000         &       0.016         &       0.914         \\
Donor FE            &           Y         &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         &           Y         \\


==> results_table/covid_on_local_giving.tex <==
\\ \multicolumn{2}{l}{\textbf{Panel A: Pooled Change After Covid}} \\ \\[-1ex]
                    &\multicolumn{1}{c}{Any Local Donation}&\multicolumn{1}{c}{Local Share (Value)}&\multicolumn{1}{c}{Local Share (Count)}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
High Covid $\times$ Post&      0.0167\sym{***}&      0.0096\sym{***}&      0.0080\sym{***}\\
                    &    (0.0044)         &    (0.0022)         &    (0.0020)         \\
\addlinespace
Low Covid $\times$ Post&      0.0022         &      0.0013         &      0.0017         \\
                    &    (0.0035)         &    (0.0015)         &    (0.0015)         \\
\midrule
Obs.                &     251,037         &     251,037         &     251,037         \\
Mean Outcome        &       0.470         &       0.173         &       0.160         \\
P(diff)             &       0.022         &       0.002         &       0.009         \\
Donor FE            &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         \\
\midrule \\ \multicolumn{2}{l}{\textbf{Panel B: Year by Year Change After Covid}} \\ \\[-1ex]
                    &\multicolumn{1}{c}{Any Local Donation}&\multicolumn{1}{c}{Local Share (Value)}&\multicolumn{1}{c}{Local Share (Count)}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
High Covid $\times$ 2020&      0.0280\sym{***}&      0.0167\sym{***}&      0.0144\sym{***}\\
                    &    (0.0050)         &    (0.0024)         &    (0.0021)         \\
\addlinespace
High Covid $\times$ 2021&     -0.0042         &     -0.0034         &     -0.0033         \\
                    &    (0.0046)         &    (0.0028)         &    (0.0026)         \\
\addlinespace
Low Covid $\times$ 2020&      0.0090\sym{**} &      0.0055\sym{***}&      0.0047\sym{***}\\
                    &    (0.0036)         &    (0.0017)         &    (0.0016)         \\
\addlinespace
Low Covid $\times$ 2021&     -0.0139\sym{***}&     -0.0086\sym{***}&     -0.0058\sym{***}\\
                    &    (0.0042)         &    (0.0017)         &    (0.0019)         \\
\midrule
Obs.                &     251,037         &     251,037         &     251,037         \\
Mean Outcome        &       0.470         &       0.173         &       0.160         \\
Donor FE            &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         \\


==> results_table/covid_on_local_giving_by_year.tex <==
                    &\multicolumn{1}{c}{Any Local Donation}&\multicolumn{1}{c}{Local Share (Value)}&\multicolumn{1}{c}{Local Share (Count)}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\hline \\ \multicolumn{2}{c}{\textbf{Panel B: Response by Year}} \\ \\[-1ex]
High Covid $\times$ 2020&      0.0280\sym{***}&      0.0167\sym{***}&      0.0144\sym{***}\\
                    &    (0.0050)         &    (0.0024)         &    (0.0021)         \\
\addlinespace
High Covid $\times$ 2021&     -0.0042         &     -0.0034         &     -0.0033         \\
                    &    (0.0046)         &    (0.0028)         &    (0.0025)         \\
\addlinespace
High Covid $\times$ 2022&      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         \\
\addlinespace
Low Covid $\times$ 2020&      0.0090\sym{**} &      0.0055\sym{***}&      0.0047\sym{***}\\
                    &    (0.0036)         &    (0.0017)         &    (0.0016)         \\
\addlinespace
Low Covid $\times$ 2021&     -0.0139\sym{***}&     -0.0086\sym{***}&     -0.0058\sym{***}\\
                    &    (0.0042)         &    (0.0017)         &    (0.0019)         \\
\addlinespace
Low Covid $\times$ 2022&      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         \\
\midrule
Obs                 &     251,043         &     251,043         &     251,043         \\
Mean Outcome        &       0.470         &       0.173         &       0.160         \\
Donor FE            &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         \\


==> results_table/covid_on_local_gshare_by_sector.tex <==
                    &\multicolumn{1}{c}{Social Services}&\multicolumn{1}{c}{Religious}&\multicolumn{1}{c}{Health/MedicalRes}&\multicolumn{1}{c}{Edu/Res/Cul}&\multicolumn{1}{c}{Environment}&\multicolumn{1}{c}{Others/Unclass}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\midrule
High GDP Impact $\times$ Post&      0.0029\sym{**} &     -0.0005         &      0.0045\sym{***}&     -0.0005         &      0.0017\sym{**} &      0.0015         \\
                    &    (0.0012)         &    (0.0010)         &    (0.0013)         &    (0.0007)         &    (0.0008)         &    (0.0013)         \\
\addlinespace
Low GDP Impact $\times$ Post&     -0.0000         &     -0.0008         &      0.0043\sym{***}&     -0.0021\sym{***}&     -0.0001         &      0.0002         \\
                    &    (0.0011)         &    (0.0009)         &    (0.0010)         &    (0.0006)         &    (0.0004)         &    (0.0007)         \\
\midrule
Obs                 &     262,648         &     262,648         &     262,648         &     262,648         &     262,648         &     262,648         \\
Mean Outcome        &       0.031         &       0.062         &       0.036         &       0.020         &       0.009         &       0.014         \\
P(diff)             &       0.066         &       0.788         &       0.879         &       0.027         &       0.038         &       0.388         \\
Share of Zero       &       0.907         &       0.901         &       0.885         &       0.951         &       0.966         &       0.956         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Donor FE            &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\


==> results_table/covid_on_local_gshare_by_sector_ns.tex <==
                    &\multicolumn{1}{c}{Social Services}&\multicolumn{1}{c}{Religious}&\multicolumn{1}{c}{Health/MedicalRes}&\multicolumn{1}{c}{Edu/Res/Cul}&\multicolumn{1}{c}{Environment}&\multicolumn{1}{c}{Others/Unclass}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\midrule
High GDP Impact $\times$ Post&      0.0041\sym{***}&     -0.0021\sym{*}  &      0.0026\sym{*}  &      0.0004         &      0.0016\sym{*}  &      0.0015         \\
                    &    (0.0012)         &    (0.0012)         &    (0.0015)         &    (0.0009)         &    (0.0008)         &    (0.0014)         \\
\addlinespace
Low GDP Impact $\times$ Post&      0.0012         &     -0.0025\sym{**} &      0.0015         &     -0.0014\sym{*}  &      0.0001         &      0.0005         \\
                    &    (0.0012)         &    (0.0011)         &    (0.0012)         &    (0.0008)         &    (0.0005)         &    (0.0008)         \\
\midrule
Obs                 &     262,648         &     262,648         &     262,648         &     262,648         &     262,648         &     262,648         \\
Mean Outcome        &       0.031         &       0.062         &       0.036         &       0.020         &       0.009         &       0.014         \\
P(diff)             &       0.094         &       0.789         &       0.514         &       0.080         &       0.100         &       0.561         \\
Share of Zero       &       0.907         &       0.901         &       0.885         &       0.951         &       0.966         &       0.956         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Donor FE            &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Sectoral Composition&           N         &           N         &           N         &           N         &           N         &           N         \\


==> results_table/covid_on_local_share.tex <==
                    &\multicolumn{1}{c}{Any Local Donation}&\multicolumn{1}{c}{Local Share (Value)}&\multicolumn{1}{c}{Local Share (Count)}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
High Covid $\times$ Post&      0.0167\sym{***}&      0.0096\sym{***}&      0.0080\sym{***}\\
                    &    (0.0044)         &    (0.0022)         &    (0.0020)         \\
\addlinespace
Low Covid $\times$ Post&      0.0022         &      0.0013         &      0.0017         \\
                    &    (0.0035)         &    (0.0015)         &    (0.0015)         \\
\midrule
Obs                 &     251,043         &     251,043         &     251,043         \\
Mean Outcome        &       0.470         &       0.173         &       0.160         \\
P(diff)             &       0.022         &       0.002         &       0.009         \\
Donor FE            &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         \\


==> results_table/covid_on_local_share1.tex <==
                    &\multicolumn{1}{c}{Any Local Donation}&\multicolumn{1}{c}{Local Share (Value)}&\multicolumn{1}{c}{Local Share (Count)}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
High Covid $\times$ Post&      0.0156\sym{***}&      0.0082\sym{***}&      0.0070\sym{***}\\
                    &    (0.0037)         &    (0.0022)         &    (0.0022)         \\
\addlinespace
Low Covid $\times$ Post&      0.0025         &      0.0019         &      0.0021         \\
                    &    (0.0030)         &    (0.0015)         &    (0.0015)         \\
\midrule
Obs                 &     251,043         &     251,043         &     251,043         \\
Mean Outcome        &       0.470         &       0.173         &       0.160         \\
P(diff)             &       0.005         &       0.012         &       0.041         \\
Donor FE            &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         \\


==> results_table/covid_on_local_share2.tex <==
                    &\multicolumn{1}{c}{Any Local Donation}&\multicolumn{1}{c}{Local Share (Value)}&\multicolumn{1}{c}{Local Share (Count)}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
High Covid $\times$ Post&      0.0092\sym{**} &      0.0043\sym{*}  &      0.0038         \\
                    &    (0.0042)         &    (0.0025)         &    (0.0024)         \\
\addlinespace
Low Covid $\times$ Post&      0.0046         &      0.0036\sym{**} &      0.0034\sym{**} \\
                    &    (0.0033)         &    (0.0015)         &    (0.0016)         \\
\midrule
Obs                 &     284,853         &     284,853         &     284,853         \\
Mean Outcome        &       0.470         &       0.175         &       0.162         \\
P(diff)             &       0.412         &       0.807         &       0.898         \\
Donor FE            &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         \\


==> results_table/covid_on_local_share2022.tex <==
                    &\multicolumn{1}{c}{Any Local Donation}&\multicolumn{1}{c}{Local Share (Value)}&\multicolumn{1}{c}{Local Share (Count)}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
High Covid $\times$ Post&      0.0092\sym{**} &      0.0043\sym{*}  &      0.0038         \\
                    &    (0.0042)         &    (0.0025)         &    (0.0024)         \\
\addlinespace
Low Covid $\times$ Post&      0.0046         &      0.0036\sym{**} &      0.0034\sym{**} \\
                    &    (0.0033)         &    (0.0015)         &    (0.0016)         \\
\midrule
Obs                 &     284,853         &     284,853         &     284,853         \\
Mean Outcome        &       0.470         &       0.175         &       0.162         \\
P(diff)             &       0.412         &       0.807         &       0.898         \\
Donor FE            &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         \\


==> results_table/covid_on_local_share3.tex <==
                    &\multicolumn{1}{c}{Any Local Donation}&\multicolumn{1}{c}{Local Share (Value)}&\multicolumn{1}{c}{Local Share (Count)}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
High Covid $\times$ Post&      0.0059         &      0.0021         &      0.0024         \\
                    &    (0.0044)         &    (0.0026)         &    (0.0025)         \\
\addlinespace
Low Covid $\times$ Post&      0.0064\sym{**} &      0.0047\sym{***}&      0.0042\sym{***}\\
                    &    (0.0028)         &    (0.0014)         &    (0.0014)         \\
\midrule
Obs                 &     284,853         &     284,853         &     284,853         \\
Mean Outcome        &       0.470         &       0.175         &       0.162         \\
P(diff)             &       0.917         &       0.360         &       0.493         \\
Donor FE            &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         \\


==> results_table/covid_on_local_share_by_sector.tex <==
                    &\multicolumn{1}{c}{Social Services}&\multicolumn{1}{c}{Religious}&\multicolumn{1}{c}{Health/MedicalRes}&\multicolumn{1}{c}{Edu/Res/Cul}&\multicolumn{1}{c}{Environment}&\multicolumn{1}{c}{Others/Unclass}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\midrule
High Covid $\times$ Post&      0.0069\sym{***}&     -0.0085\sym{**} &      0.0191\sym{***}&     -0.0039         &      0.0094\sym{*}  &      0.0062         \\
                    &    (0.0022)         &    (0.0038)         &    (0.0046)         &    (0.0061)         &    (0.0050)         &    (0.0042)         \\
\addlinespace
Low Covid $\times$ Post&      0.0016         &     -0.0066\sym{*}  &      0.0168\sym{***}&     -0.0104\sym{**} &      0.0046         &      0.0037         \\
                    &    (0.0019)         &    (0.0038)         &    (0.0031)         &    (0.0050)         &    (0.0034)         &    (0.0033)         \\
\midrule
Obs                 &     196,482         &      86,296         &     138,464         &      55,458         &      56,565         &     103,779         \\
Mean Outcome        &       0.074         &       0.344         &       0.179         &       0.252         &       0.141         &       0.110         \\
P(diff)             &       0.062         &       0.677         &       0.657         &       0.347         &       0.430         &       0.650         \\
Donor FE            &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\


==> results_table/covid_on_local_share_by_year.tex <==
                    &\multicolumn{1}{c}{Any Local Donation}&\multicolumn{1}{c}{Local Share (Value)}&\multicolumn{1}{c}{Local Share (Count)}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
High Covid $\times$ 2020&      0.0280\sym{***}&      0.0167\sym{***}&      0.0144\sym{***}\\
                    &    (0.0050)         &    (0.0024)         &    (0.0021)         \\
\addlinespace
High Covid $\times$ 2021&     -0.0042         &     -0.0034         &     -0.0033         \\
                    &    (0.0046)         &    (0.0028)         &    (0.0025)         \\
\addlinespace
High Covid $\times$ 2022&      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         \\
\addlinespace
Low Covid $\times$ 2020&      0.0090\sym{**} &      0.0055\sym{***}&      0.0047\sym{***}\\
                    &    (0.0036)         &    (0.0017)         &    (0.0016)         \\
\addlinespace
Low Covid $\times$ 2021&     -0.0139\sym{***}&     -0.0086\sym{***}&     -0.0058\sym{***}\\
                    &    (0.0042)         &    (0.0017)         &    (0.0019)         \\
\addlinespace
Low Covid $\times$ 2022&      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         \\
\midrule
Obs                 &     251,043         &     251,043         &     251,043         \\
Mean Outcome        &       0.470         &       0.173         &       0.160         \\
Donor FE            &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         \\


==> results_table/covid_on_local_share_by_year1.tex <==
                    &\multicolumn{1}{c}{Any Local Donation}&\multicolumn{1}{c}{Local Share (Value)}&\multicolumn{1}{c}{Local Share (Count)}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
High Covid $\times$ 2020&      0.0175\sym{***}&      0.0110\sym{***}&      0.0099\sym{***}\\
                    &    (0.0040)         &    (0.0023)         &    (0.0024)         \\
\addlinespace
High Covid $\times$ 2021&     -0.0005         &     -0.0050\sym{*}  &     -0.0047\sym{*}  \\
                    &    (0.0057)         &    (0.0028)         &    (0.0026)         \\
\addlinespace
High Covid $\times$ 2022&      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         \\
\addlinespace
Low Covid $\times$ 2020&      0.0141\sym{***}&      0.0081\sym{***}&      0.0067\sym{***}\\
                    &    (0.0035)         &    (0.0017)         &    (0.0016)         \\
\addlinespace
Low Covid $\times$ 2021&     -0.0137\sym{***}&     -0.0074\sym{***}&     -0.0051\sym{***}\\
                    &    (0.0036)         &    (0.0019)         &    (0.0019)         \\
\addlinespace
Low Covid $\times$ 2022&      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         \\
\midrule
Obs                 &     251,043         &     251,043         &     251,043         \\
Mean Outcome        &       0.470         &       0.173         &       0.160         \\
Donor FE            &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         \\


==> results_table/covid_on_local_share_by_year2.tex <==
                    &\multicolumn{1}{c}{Any Local Donation}&\multicolumn{1}{c}{Local Share (Value)}&\multicolumn{1}{c}{Local Share (Count)}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
High Covid $\times$ 2020&      0.0277\sym{***}&      0.0166\sym{***}&      0.0143\sym{***}\\
                    &    (0.0050)         &    (0.0024)         &    (0.0021)         \\
\addlinespace
High Covid $\times$ 2021&     -0.0039         &     -0.0034         &     -0.0032         \\
                    &    (0.0046)         &    (0.0027)         &    (0.0025)         \\
\addlinespace
High Covid $\times$ 2022&     -0.0092         &     -0.0059         &     -0.0040         \\
                    &    (0.0077)         &    (0.0051)         &    (0.0047)         \\
\addlinespace
Low Covid $\times$ 2020&      0.0079\sym{**} &      0.0051\sym{***}&      0.0044\sym{***}\\
                    &    (0.0036)         &    (0.0017)         &    (0.0017)         \\
\addlinespace
Low Covid $\times$ 2021&     -0.0153\sym{***}&     -0.0088\sym{***}&     -0.0061\sym{***}\\
                    &    (0.0043)         &    (0.0018)         &    (0.0019)         \\
\addlinespace
Low Covid $\times$ 2022&      0.0122         &      0.0117\sym{**} &      0.0102\sym{**} \\
                    &    (0.0079)         &    (0.0054)         &    (0.0045)         \\
\midrule
Obs                 &     284,853         &     284,853         &     284,853         \\
Mean Outcome        &       0.470         &       0.175         &       0.162         \\
Donor FE            &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         \\


==> results_table/covid_on_local_share_by_year2022.tex <==
                    &\multicolumn{1}{c}{Any Local Donation}&\multicolumn{1}{c}{Local Share (Value)}&\multicolumn{1}{c}{Local Share (Count)}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
High Covid $\times$ 2020&      0.0280\sym{***}&      0.0167\sym{***}&      0.0144\sym{***}\\
                    &    (0.0050)         &    (0.0024)         &    (0.0021)         \\
\addlinespace
High Covid $\times$ 2021&     -0.0042         &     -0.0034         &     -0.0033         \\
                    &    (0.0046)         &    (0.0028)         &    (0.0025)         \\
\addlinespace
High Covid $\times$ 2022&      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         \\
\addlinespace
Low Covid $\times$ 2020&      0.0090\sym{**} &      0.0055\sym{***}&      0.0047\sym{***}\\
                    &    (0.0036)         &    (0.0017)         &    (0.0016)         \\
\addlinespace
Low Covid $\times$ 2021&     -0.0139\sym{***}&     -0.0086\sym{***}&     -0.0058\sym{***}\\
                    &    (0.0042)         &    (0.0017)         &    (0.0019)         \\
\addlinespace
Low Covid $\times$ 2022&      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         \\
\midrule
Obs                 &     251,043         &     251,043         &     251,043         \\
Mean Outcome        &       0.470         &       0.173         &       0.160         \\
Donor FE            &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         \\


==> results_table/covid_on_local_share_by_year3.tex <==
                    &\multicolumn{1}{c}{Any Local Donation}&\multicolumn{1}{c}{Local Share (Value)}&\multicolumn{1}{c}{Local Share (Count)}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
High Covid $\times$ 2020&      0.0180\sym{***}&      0.0113\sym{***}&      0.0101\sym{***}\\
                    &    (0.0041)         &    (0.0025)         &    (0.0024)         \\
\addlinespace
High Covid $\times$ 2021&      0.0017         &     -0.0027         &     -0.0027         \\
                    &    (0.0055)         &    (0.0029)         &    (0.0027)         \\
\addlinespace
High Covid $\times$ 2022&     -0.0135\sym{**} &     -0.0082\sym{**} &     -0.0055         \\
                    &    (0.0058)         &    (0.0038)         &    (0.0035)         \\
\addlinespace
Low Covid $\times$ 2020&      0.0125\sym{***}&      0.0075\sym{***}&      0.0062\sym{***}\\
                    &    (0.0036)         &    (0.0017)         &    (0.0016)         \\
\addlinespace
Low Covid $\times$ 2021&     -0.0154\sym{***}&     -0.0082\sym{***}&     -0.0058\sym{***}\\
                    &    (0.0036)         &    (0.0017)         &    (0.0018)         \\
\addlinespace
Low Covid $\times$ 2022&      0.0217\sym{**} &      0.0185\sym{***}&      0.0153\sym{***}\\
                    &    (0.0097)         &    (0.0066)         &    (0.0054)         \\
\midrule
Obs                 &     284,853         &     284,853         &     284,853         \\
Mean Outcome        &       0.470         &       0.175         &       0.162         \\
Donor FE            &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         \\


==> results_table/covid_on_sectoral_share.tex <==
                    &\multicolumn{1}{c}{Social Services}&\multicolumn{1}{c}{Religious}&\multicolumn{1}{c}{Health/MedicalRes}&\multicolumn{1}{c}{Edu/Res/Cul}&\multicolumn{1}{c}{Environment}&\multicolumn{1}{c}{Others/Unclass}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\midrule
High Covid $\times$ Post&      0.0109\sym{***}&     -0.0038\sym{***}&     -0.0087\sym{***}&      0.0023\sym{*}  &     -0.0006         &     -0.0001         \\
                    &    (0.0020)         &    (0.0014)         &    (0.0026)         &    (0.0013)         &    (0.0011)         &    (0.0018)         \\
\addlinespace
Low Covid $\times$ Post&      0.0120\sym{***}&     -0.0040\sym{***}&     -0.0127\sym{***}&      0.0017         &      0.0010         &      0.0021         \\
                    &    (0.0021)         &    (0.0013)         &    (0.0020)         &    (0.0014)         &    (0.0008)         &    (0.0014)         \\
\midrule
Obs                 &     251,043         &     251,043         &     251,043         &     251,043         &     251,043         &     251,043         \\
Mean Outcome        &       0.427         &       0.158         &       0.189         &       0.062         &       0.060         &       0.105         \\
Share of Zero       &       0.212         &       0.642         &       0.432         &       0.753         &       0.752         &       0.563         \\
P(diff)             &       0.672         &       0.909         &       0.106         &       0.668         &       0.200         &       0.278         \\
Donor FE            &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\


==> results_table/determinants_local_giving.tex <==
            &\multicolumn{3}{c}{Any Local Donation}                           &\multicolumn{3}{c}{Local Share (Value)}                          \\\cmidrule(lr){2-4}\cmidrule(lr){5-7}
            &   LPM (All)         &LPM (Don Count ≥ 5)         &       Tobit         &   LPM (All)         &LPM (Don Count ≥ 5)         &       Tobit         \\
\midrule
main        &                     &                     &                     &                     &                     &                     \\
Male        &      -0.004         &       0.003         &      -0.004         &       0.006\sym{**} &       0.005         &       0.006\sym{**} \\
            &     (0.005)         &     (0.007)         &     (0.005)         &     (0.003)         &     (0.003)         &     (0.003)         \\
\addlinespace
Wealth Index&       0.000\sym{**} &       0.001\sym{***}&       0.000\sym{**} &       0.000\sym{***}&       0.000\sym{***}&       0.000\sym{***}\\
            &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         \\
\addlinespace
Urban       &       0.029\sym{***}&       0.034\sym{***}&       0.029\sym{***}&       0.014\sym{***}&       0.015\sym{***}&       0.014\sym{***}\\
            &     (0.006)         &     (0.008)         &     (0.006)         &     (0.003)         &     (0.004)         &     (0.003)         \\
\addlinespace
Level-4 Qual. (\%)&       0.001\sym{*}  &       0.001\sym{***}&       0.001\sym{*}  &       0.000         &       0.000\sym{*}  &       0.000         \\
            &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         \\
\addlinespace
Age 65+ (\%)&       0.000         &       0.000         &       0.000         &      -0.000\sym{**} &      -0.000\sym{**} &      -0.000\sym{**} \\
            &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         \\
\addlinespace
British White (\%)&      -0.000         &      -0.000         &      -0.000         &      -0.000         &      -0.000         &      -0.000         \\
            &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         \\
\addlinespace
Religious (\%)&       0.000         &       0.000         &       0.000         &      -0.000         &      -0.000\sym{**} &      -0.000         \\
            &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         \\
\addlinespace
Self-claim UK Identity (\%)&       0.002\sym{***}&       0.002\sym{***}&       0.002\sym{***}&       0.001\sym{***}&       0.001\sym{***}&       0.001\sym{***}\\
            &     (0.000)         &     (0.001)         &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         \\
\addlinespace
Conservative Vote Share&       0.100         &       0.130         &       0.100         &      -0.021         &       0.009         &      -0.021         \\
            &     (0.083)         &     (0.109)         &     (0.083)         &     (0.042)         &     (0.047)         &     (0.042)         \\
\addlinespace
Labour Vote Share&       0.139\sym{*}  &       0.146         &       0.139\sym{*}  &       0.057         &       0.080\sym{*}  &       0.057         \\
            &     (0.083)         &     (0.108)         &     (0.083)         &     (0.042)         &     (0.045)         &     (0.042)         \\
\addlinespace
LibDem Vote Share&       0.168\sym{**} &       0.191\sym{*}  &       0.168\sym{**} &       0.072\sym{*}  &       0.090\sym{**} &       0.072\sym{*}  \\
            &     (0.076)         &     (0.098)         &     (0.076)         &     (0.038)         &     (0.040)         &     (0.038)         \\
\addlinespace
High Hate-Crime Area&      -0.013         &      -0.017         &      -0.013         &      -0.004         &      -0.005         &      -0.004         \\
            &     (0.009)         &     (0.011)         &     (0.009)         &     (0.005)         &     (0.005)         &     (0.005)         \\
\addlinespace
Ethnic Homogeneity&       0.142\sym{*}  &       0.084         &       0.142\sym{*}  &       0.157\sym{***}&       0.162\sym{***}&       0.157\sym{***}\\
            &     (0.079)         &     (0.087)         &     (0.079)         &     (0.047)         &     (0.046)         &     (0.047)         \\
\midrule
Obs         &     175,091         &     112,180         &     175,091         &     175,091         &     112,180         &     175,091         \\
Sectoral Composition&           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Year FEs    &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\


==> results_table/differential_response_decappeal.tex <==
                    &\multicolumn{5}{c}{Giving to Dec Appeal Charities (0/1)}                                                     \\\cmidrule(lr){2-6}
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
                    &\multicolumn{1}{c}{All Appeals}&\multicolumn{1}{c}{Covid Appeal}&\multicolumn{1}{c}{Afghanistan Crisis}&\multicolumn{1}{c}{Ukraine Appeal}&\multicolumn{1}{c}{Pakistan Floods}\\
\midrule
DEC Appeal          &      0.0161\sym{***}&      0.0167\sym{***}&      0.0163\sym{***}&      0.0177\sym{***}&      0.0167\sym{***}\\
                    &    (0.0008)         &    (0.0008)         &    (0.0008)         &    (0.0008)         &    (0.0008)         \\
\addlinespace
DEC Appeal $\times$ Post Covid&      0.0035\sym{***}&     -0.0154\sym{***}&      0.0145\sym{***}&      0.0188\sym{***}&     -0.0065\sym{***}\\
                    &    (0.0006)         &    (0.0009)         &    (0.0009)         &    (0.0009)         &    (0.0009)         \\
\addlinespace
DEC Appeal $\times$ High Covid $\times$ Post Covid&     -0.0029\sym{***}&     -0.0026\sym{*}  &     -0.0030\sym{**} &     -0.0021         &     -0.0029\sym{**} \\
                    &    (0.0010)         &    (0.0014)         &    (0.0014)         &    (0.0016)         &    (0.0013)         \\
\midrule
Obs.                &   6,173,952         &   6,173,952         &   6,173,952         &   6,173,952         &   6,173,952         \\
Post Covid          &           Y         &           Y         &           Y         &           Y         &           Y         \\
High Covid $\times$ Post Covid&           Y         &           Y         &           Y         &           Y         &           Y         \\
Dec Appeal $\times$ High Covid&           Y         &           Y         &           Y         &           Y         &           Y         \\
Donor Fixed Effects &           Y         &           Y         &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         &           Y         \\
Month Fixed Effects &           Y         &           Y         &           Y         &           Y         &           Y         \\
Total Monthly Donation&           Y         &           Y         &           Y         &           Y         &           Y         \\


==> results_table/distribution_of_distance_to_local_charities.tex <==
                    &\multicolumn{1}{c}{Share by Donation Count (\%)}&\multicolumn{1}{c}{Cumulative Share by Count (\%)}&\multicolumn{1}{c}{Share by Donation Value (\%)}&\multicolumn{1}{c}{Cumulative Share by Value (\%)}\\
\hline
Donor within charity area&       58.95&       58.95&       56.55&       56.55\\
0 $<$ d $\leq$ 10 km&       10.98&       69.93&       14.31&       70.86\\
10 $<$ d $\leq$ 25 km&        4.84&       74.77&        4.76&       75.62\\
25 $<$ d $\leq$ 50 km&        5.19&       79.96&        6.06&       81.68\\
50 $<$ d $\leq$ 100 km&        7.52&       87.48&        7.21&       88.89\\
100 $<$ d $\leq$ 150 km&        4.03&       91.51&        3.38&       92.27\\
150 $<$ d $\leq$ 200 km&        3.02&       94.53&        2.97&       95.25\\
d $>$ 200 km        &        5.47&      100.00&        4.75&      100.00\\


==> results_table/gdp_on_geo_composition_value.tex <==
                    &\multicolumn{1}{c}{Local Share}&\multicolumn{1}{c}{National Share}&\multicolumn{1}{c}{Nat/Overseas Share}&\multicolumn{1}{c}{Overseas Share}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\midrule
High GDP Hit $\times$ Post&      0.0010         &     -0.0099\sym{***}&      0.0063\sym{***}&      0.0026\sym{**} \\
                    &    (0.0019)         &    (0.0026)         &    (0.0014)         &    (0.0011)         \\
\addlinespace
Low GDP Hit $\times$ Post&      0.0081\sym{***}&     -0.0172\sym{***}&      0.0047\sym{***}&      0.0044\sym{***}\\
                    &    (0.0020)         &    (0.0024)         &    (0.0015)         &    (0.0011)         \\
\midrule
Obs                 &     251,043         &     251,043         &     251,043         &     251,043         \\
Mean Outcome        &       0.173         &       0.482         &       0.218         &       0.127         \\
P(diff)             &       0.009         &       0.040         &       0.345         &       0.269         \\
Donor FE            &           Y         &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         &           Y         \\


==> results_table/gdp_on_local_giving.tex <==
                    &\multicolumn{1}{c}{Any Local Donation}&\multicolumn{1}{c}{Local Share (Value)}&\multicolumn{1}{c}{Local Share (Count)}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Large GDP Shock $\times$ Post&     -0.0044         &     -0.0015         &     -0.0006         \\
                    &    (0.0044)         &    (0.0018)         &    (0.0018)         \\
\addlinespace
Small GDP Shock $\times$ Post&      0.0151\sym{***}&      0.0080\sym{***}&      0.0069\sym{***}\\
                    &    (0.0033)         &    (0.0018)         &    (0.0017)         \\
\midrule
Obs.                &     251,037         &     251,037         &     251,037         \\
Mean outcome        &       0.470         &       0.173         &       0.160         \\
P(Diff)             &       0.002         &       0.000         &       0.002         \\
Donor FE            &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         \\


==> results_table/gdp_on_local_share.tex <==
                    &\multicolumn{1}{c}{Any Local Donation}&\multicolumn{1}{c}{Local Share (Value)}&\multicolumn{1}{c}{Local Share (Count)}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
High GDP Hit $\times$ Post&     -0.0008         &      0.0010         &      0.0015         \\
                    &    (0.0040)         &    (0.0019)         &    (0.0019)         \\
\addlinespace
Low GDP Hit $\times$ Post&      0.0172\sym{***}&      0.0081\sym{***}&      0.0068\sym{***}\\
                    &    (0.0039)         &    (0.0020)         &    (0.0019)         \\
\midrule
Obs                 &     251,043         &     251,043         &     251,043         \\
Mean Outcome        &       0.470         &       0.173         &       0.160         \\
P(diff)             &       0.003         &       0.009         &       0.036         \\
Donor FE            &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         \\


==> results_table/gdp_on_local_share_by_sector.tex <==
                    &\multicolumn{1}{c}{Social Services}&\multicolumn{1}{c}{Religious}&\multicolumn{1}{c}{Health/MedicalRes}&\multicolumn{1}{c}{Edu/Res/Cul}&\multicolumn{1}{c}{Environment}&\multicolumn{1}{c}{Others/Unclass}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\midrule
High GDP Hit $\times$ Post&      0.0017         &     -0.0071\sym{*}  &      0.0156\sym{***}&     -0.0082         &      0.0040         &      0.0002         \\
                    &    (0.0022)         &    (0.0037)         &    (0.0036)         &    (0.0058)         &    (0.0036)         &    (0.0035)         \\
\addlinespace
Low GDP Hit $\times$ Post&      0.0055\sym{***}&     -0.0074\sym{*}  &      0.0201\sym{***}&     -0.0088\sym{*}  &      0.0088\sym{**} &      0.0100\sym{***}\\
                    &    (0.0019)         &    (0.0038)         &    (0.0041)         &    (0.0053)         &    (0.0042)         &    (0.0033)         \\
\midrule
Obs                 &     196,482         &      86,296         &     138,464         &      55,458         &      56,565         &     103,779         \\
Mean Outcome        &       0.074         &       0.344         &       0.179         &       0.252         &       0.141         &       0.110         \\
P(diff)             &       0.177         &       0.952         &       0.381         &       0.936         &       0.369         &       0.030         \\
Donor FE            &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\


==> results_table/gdpdrop_on_local_share.tex <==
                    &\multicolumn{1}{c}{Any Donation}&\multicolumn{2}{c}{Any Local}              &\multicolumn{2}{c}{Local Share (Value)}    &\multicolumn{2}{c}{Local Share (Number)}   \\\cmidrule(lr){2-2}\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}\\
                    &\multicolumn{1}{c}{Full}&\multicolumn{1}{c}{Full}&\multicolumn{1}{c}{Total $>$ 0}&\multicolumn{1}{c}{Full}&\multicolumn{1}{c}{Total $>$ 0}&\multicolumn{1}{c}{Full}&\multicolumn{1}{c}{Total $>$ 0}\\
\midrule
High GDP Impact $\times$ Post&     -0.0069\sym{***}&      0.0029         &      0.0052         &      0.0017         &      0.0034         &      0.0016         &      0.0039\sym{*}  \\
                    &    (0.0010)         &    (0.0026)         &    (0.0043)         &    (0.0013)         &    (0.0021)         &    (0.0014)         &    (0.0021)         \\
\addlinespace
Low GDP Impact $\times$ Post&     -0.0073\sym{***}&      0.0049\sym{*}  &      0.0089\sym{*}  &      0.0026\sym{*}  &      0.0049\sym{**} &      0.0021         &      0.0038\sym{*}  \\
                    &    (0.0010)         &    (0.0030)         &    (0.0046)         &    (0.0015)         &    (0.0022)         &    (0.0014)         &    (0.0021)         \\
\midrule
Obs                 &     423,423         &     423,423         &     262,648         &     423,423         &     262,648         &     423,423         &     262,648         \\
Mean Outcome        &         .62         &        .292         &         .47         &        .107         &        .173         &        .099         &         .16         \\
P(diff)             &        .789         &        .644         &        .592         &        .659         &        .608         &        .833         &        .961         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Donor FE            &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Sectoral Composition&                     &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\


==> results_table/hatecrime_on_local_giving.tex <==
\\ \multicolumn{2}{l}{\textbf{Panel A:}} \\
                    &\multicolumn{1}{c}{Any Local Donation}&\multicolumn{1}{c}{Local Share (Value)}&\multicolumn{1}{c}{Local Share (Count)}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Low Hate-crime $\times$ Post&      0.0208\sym{***}&      0.0096\sym{***}&      0.0081\sym{***}\\
                    &    (0.0032)         &    (0.0017)         &    (0.0017)         \\
\addlinespace
High Hate-crime $\times$ Post&     -0.0106\sym{**} &     -0.0029         &     -0.0018         \\
                    &    (0.0047)         &    (0.0019)         &    (0.0018)         \\
\midrule \\ \multicolumn{2}{l}{\textbf{Panel B:}} \\ 
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Low Ethnic Homogeneity $\times$ Post&     -0.0051         &     -0.0013         &     -0.0006         \\
                    &    (0.0049)         &    (0.0023)         &    (0.0022)         \\
\addlinespace
High Ethnic Homogeneity $\times$ Post&      0.0191\sym{***}&      0.0094\sym{***}&      0.0082\sym{***}\\
                    &    (0.0038)         &    (0.0018)         &    (0.0017)         \\
\midrule \\ \multicolumn{2}{l}{\textbf{Panel C:}} \\
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Low Local Belonging $\times$ Post&     -0.0036         &     -0.0022         &     -0.0011         \\
                    &    (0.0053)         &    (0.0022)         &    (0.0022)         \\
\addlinespace
High Local Belonging $\times$ Post&      0.0127\sym{***}&      0.0074\sym{***}&      0.0064\sym{***}\\
                    &    (0.0026)         &    (0.0015)         &    (0.0015)         \\
\midrule
Obs                 &     251,037         &     251,037         &     251,037         \\
Mean outcome        &       0.470         &       0.173         &       0.160         \\
P(Diff)             &       0.009         &       0.000         &       0.002         \\
Donor FE            &           Y         &           Y         &           Y         \\
Year trend          &           Y         &           Y         &           Y         \\
Total donation control&           Y         &           Y         &           Y         \\
Sectoral composition controls&           Y         &           Y         &           Y         \\


==> results_table/heterogeneities.tex <==
                    &\multicolumn{5}{c}{Local Share (Value)}                                                                      \\\cmidrule(lr){2-6}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         \\
\midrule
Post-Covid          &      0.0004         &      0.0075         &     -0.0043         &      0.0009         &      0.0061         \\
                    &    (0.0057)         &    (0.0050)         &    (0.0056)         &    (0.0051)         &    (0.0055)         \\
\addlinespace
Post-Covid $\times$ High Covid&      0.0082\sym{***}&                     &                     &                     &                     \\
                    &    (0.0027)         &                     &                     &                     &                     \\
\addlinespace
Post-Covid $\times$ High Hate Crime Rate&                     &     -0.0154\sym{***}&                     &                     &                     \\
                    &                     &    (0.0023)         &                     &                     &                     \\
\addlinespace
Post-Covid $\times$ More Culturally Homogeneous&                     &                     &      0.0115\sym{***}&                     &                     \\
                    &                     &                     &    (0.0026)         &                     &                     \\
\addlinespace
Post-Covid $\times$ Stronger Sense of Local Belonging&                     &                     &                     &      0.0099\sym{***}&                     \\
                    &                     &                     &                     &    (0.0024)         &                     \\
\addlinespace
Post-Covid $\times$ Local Area Important to Identity&                     &                     &                     &                     &      0.0017         \\
                    &                     &                     &                     &                     &    (0.0023)         \\
\midrule
Obs                 &     243,251         &     243,251         &     243,251         &     243,251         &     243,251         \\
Donor Fixed Effects &           Y         &           Y         &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         &           Y         \\
Total Donations     &           Y         &           Y         &           Y         &           Y         &           Y         \\
Sectoral Composition Controls&           Y         &           Y         &           Y         &           Y         &           Y         \\
Differential Effects by Other Socio-Economic Variables&                     &                     &                     &                     &                     \\


==> results_table/heterogeneities_wcontrols.tex <==
                    &\multicolumn{5}{c}{Local Share (Value)}                                                                      \\\cmidrule(lr){2-6}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         \\
\midrule
Post-Covid          &      0.0013         &     -0.0052\sym{**} &     -0.0022         &     -0.0043\sym{**} &     -0.0024         \\
                    &    (0.0015)         &    (0.0024)         &    (0.0019)         &    (0.0021)         &    (0.0021)         \\
\addlinespace
Post-Covid $\times$ High Covid&      0.0083\sym{***}&      0.0086\sym{***}&      0.0070\sym{***}&      0.0059\sym{**} &      0.0056\sym{*}  \\
                    &    (0.0026)         &    (0.0024)         &    (0.0025)         &    (0.0023)         &    (0.0029)         \\
\addlinespace
Post-Covid $\times$ Stronger Sense of Local Belonging&                     &      0.0098\sym{***}&                     &                     &                     \\
                    &                     &    (0.0024)         &                     &                     &                     \\
\addlinespace
Post-Covid $\times$ High Neighbourhood Cohesion&                     &                     &      0.0076\sym{***}&                     &                     \\
                    &                     &                     &    (0.0027)         &                     &                     \\
\addlinespace
Post-Covid $\times$ Low Hate Crime Rate&                     &                     &                     &      0.0113\sym{***}&                     \\
                    &                     &                     &                     &    (0.0023)         &                     \\
\addlinespace
Post-Covid $\times$ More Culturally Homogeneous&                     &                     &                     &                     &      0.0092\sym{***}\\
                    &                     &                     &                     &                     &    (0.0026)         \\
\midrule
Obs                 &     251,043         &     251,043         &     251,043         &     251,043         &     251,043         \\
Donor Fixed Effects &           Y         &           Y         &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         &           Y         \\
Total Donations     &           Y         &           Y         &           Y         &           Y         &           Y         \\
Sectoral Composition Controls&           Y         &           Y         &           Y         &           Y         &           Y         \\
Differential Effects by Other Socio-Economic Variables&           N         &           N         &           N         &           N         &           N         \\


==> results_table/heterogeneities_wcontrols1.tex <==
                    &\multicolumn{5}{c}{Local Share (Value)}                                                                      \\\cmidrule(lr){2-6}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         \\
\midrule
Post-Covid          &      0.0013         &     -0.0052\sym{**} &     -0.0022         &     -0.0043\sym{**} &     -0.0024         \\
                    &    (0.0015)         &    (0.0024)         &    (0.0019)         &    (0.0021)         &    (0.0021)         \\
\addlinespace
Post-Covid $\times$ High Covid&      0.0083\sym{***}&      0.0086\sym{***}&      0.0070\sym{***}&      0.0059\sym{**} &      0.0056\sym{*}  \\
                    &    (0.0026)         &    (0.0024)         &    (0.0025)         &    (0.0023)         &    (0.0029)         \\
\addlinespace
Post-Covid $\times$ Stronger Sense of Local Belonging&                     &      0.0098\sym{***}&                     &                     &                     \\
                    &                     &    (0.0024)         &                     &                     &                     \\
\addlinespace
Post-Covid $\times$ High Neighbourhood Cohesion&                     &                     &      0.0076\sym{***}&                     &                     \\
                    &                     &                     &    (0.0027)         &                     &                     \\
\addlinespace
Post-Covid $\times$ Low Hate Crime Rate&                     &                     &                     &      0.0113\sym{***}&                     \\
                    &                     &                     &                     &    (0.0023)         &                     \\
\addlinespace
Post-Covid $\times$ More Culturally Homogeneous&                     &                     &                     &                     &      0.0092\sym{***}\\
                    &                     &                     &                     &                     &    (0.0026)         \\
\midrule
Obs                 &     251,043         &     251,043         &     251,043         &     251,043         &     251,043         \\
Donor Fixed Effects &           Y         &           Y         &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         &           Y         \\
Total Donations     &           Y         &           Y         &           Y         &           Y         &           Y         \\
Sectoral Composition Controls&           Y         &           Y         &           Y         &           Y         &           Y         \\
Differential Effects by Other Socio-Economic Variables&           N         &           N         &           N         &           N         &           N         \\


==> results_table/heterogeneities_wcontrols2.tex <==
                    &\multicolumn{5}{c}{Local Share (Value)}                                                                      \\\cmidrule(lr){2-6}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         \\
\midrule
Post-Covid          &      0.0036\sym{**} &      0.0013         &      0.0040\sym{**} &      0.0038\sym{**} &      0.0050\sym{***}\\
                    &    (0.0015)         &    (0.0023)         &    (0.0018)         &    (0.0019)         &    (0.0019)         \\
\addlinespace
Post-Covid $\times$ High Covid&      0.0007         &      0.0008         &      0.0009         &      0.0008         &      0.0018         \\
                    &    (0.0029)         &    (0.0029)         &    (0.0028)         &    (0.0029)         &    (0.0029)         \\
\addlinespace
Post-Covid $\times$ Stronger Sense of Local Belonging&                     &      0.0034         &                     &                     &                     \\
                    &                     &    (0.0023)         &                     &                     &                     \\
\addlinespace
Post-Covid $\times$ High Neighbourhood Cohesion&                     &                     &     -0.0010         &                     &                     \\
                    &                     &                     &    (0.0023)         &                     &                     \\
\addlinespace
Post-Covid $\times$ Low Hate Crime Rate&                     &                     &                     &     -0.0006         &                     \\
                    &                     &                     &                     &    (0.0026)         &                     \\
\addlinespace
Post-Covid $\times$ More Culturally Homogeneous&                     &                     &                     &                     &     -0.0036         \\
                    &                     &                     &                     &                     &    (0.0026)         \\
\midrule
Obs                 &     284,853         &     284,853         &     284,853         &     284,853         &     284,853         \\
Donor Fixed Effects &           Y         &           Y         &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         &           Y         \\
Total Donations     &           Y         &           Y         &           Y         &           Y         &           Y         \\
Sectoral Composition Controls&           Y         &           Y         &           Y         &           Y         &           Y         \\
Differential Effects by Other Socio-Economic Variables&           N         &           N         &           N         &           N         &           N         \\


==> results_table/heterogeneities_wcontrols3.tex <==
                    &\multicolumn{5}{c}{Local Share (Value)}                                                                      \\\cmidrule(lr){2-6}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         \\
\midrule
Post-Covid          &      0.0036\sym{**} &      0.0013         &      0.0040\sym{**} &      0.0038\sym{**} &      0.0050\sym{***}\\
                    &    (0.0015)         &    (0.0023)         &    (0.0018)         &    (0.0019)         &    (0.0019)         \\
\addlinespace
Post-Covid $\times$ High Covid&      0.0007         &      0.0008         &      0.0009         &      0.0008         &      0.0018         \\
                    &    (0.0029)         &    (0.0029)         &    (0.0028)         &    (0.0029)         &    (0.0029)         \\
\addlinespace
Post-Covid $\times$ Stronger Sense of Local Belonging&                     &      0.0034         &                     &                     &                     \\
                    &                     &    (0.0023)         &                     &                     &                     \\
\addlinespace
Post-Covid $\times$ High Neighbourhood Cohesion&                     &                     &     -0.0010         &                     &                     \\
                    &                     &                     &    (0.0023)         &                     &                     \\
\addlinespace
Post-Covid $\times$ Low Hate Crime Rate&                     &                     &                     &     -0.0006         &                     \\
                    &                     &                     &                     &    (0.0026)         &                     \\
\addlinespace
Post-Covid $\times$ More Culturally Homogeneous&                     &                     &                     &                     &     -0.0036         \\
                    &                     &                     &                     &                     &    (0.0026)         \\
\midrule
Obs                 &     284,853         &     284,853         &     284,853         &     284,853         &     284,853         \\
Donor Fixed Effects &           Y         &           Y         &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         &           Y         \\
Total Donations     &           Y         &           Y         &           Y         &           Y         &           Y         \\
Sectoral Composition Controls&           Y         &           Y         &           Y         &           Y         &           Y         \\
Differential Effects by Other Socio-Economic Variables&           N         &           N         &           N         &           N         &           N         \\


==> results_table/heterogeneities_wocontrols.tex <==
                    &\multicolumn{4}{c}{Local Share (Value)}                                                \\\cmidrule(lr){2-5}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\midrule
Post-Covid          &     -0.0136         &     -0.0087         &     -0.0105         &     -0.0129         \\
                    &    (0.0091)         &    (0.0094)         &    (0.0090)         &    (0.0094)         \\
\addlinespace
Post-Covid $\times$ High Covid&      0.0074\sym{***}&      0.0064\sym{**} &      0.0054\sym{**} &      0.0053         \\
                    &    (0.0027)         &    (0.0027)         &    (0.0024)         &    (0.0032)         \\
\addlinespace
Post-Covid $\times$ Stronger Sense of Local Belonging&      0.0090\sym{***}&                     &                     &                     \\
                    &    (0.0025)         &                     &                     &                     \\
\addlinespace
Post-Covid $\times$ High Neighbourhood Cohesion&                     &      0.0058\sym{*}  &                     &                     \\
                    &                     &    (0.0031)         &                     &                     \\
\addlinespace
Post-Covid $\times$ Low Hate Crime Rate&                     &                     &      0.0114\sym{***}&                     \\
                    &                     &                     &    (0.0024)         &                     \\
\addlinespace
Post-Covid $\times$ More Culturally Homogeneous&                     &                     &                     &      0.0106\sym{***}\\
                    &                     &                     &                     &    (0.0032)         \\
\midrule
Obs                 &     243,251         &     243,251         &     243,251         &     243,251         \\
Donor Fixed Effects &           Y         &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         \\
Total Donations     &           Y         &           Y         &           Y         &           Y         \\
Sectoral Composition Controls&           Y         &           Y         &           Y         &           Y         \\
Differential Effects by Other Socio-Economic Variables&           Y         &           Y         &           Y         &           Y         \\


==> results_table/heterogeneities_wocontrols1.tex <==
                    &\multicolumn{4}{c}{Local Share (Value)}                                                \\\cmidrule(lr){2-5}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\midrule
Post-Covid          &     -0.0136         &     -0.0087         &     -0.0105         &     -0.0129         \\
                    &    (0.0091)         &    (0.0094)         &    (0.0090)         &    (0.0094)         \\
\addlinespace
Post-Covid $\times$ High Covid&      0.0074\sym{***}&      0.0064\sym{**} &      0.0054\sym{**} &      0.0053         \\
                    &    (0.0027)         &    (0.0027)         &    (0.0024)         &    (0.0032)         \\
\addlinespace
Post-Covid $\times$ Stronger Sense of Local Belonging&      0.0090\sym{***}&                     &                     &                     \\
                    &    (0.0025)         &                     &                     &                     \\
\addlinespace
Post-Covid $\times$ High Neighbourhood Cohesion&                     &      0.0058\sym{*}  &                     &                     \\
                    &                     &    (0.0031)         &                     &                     \\
\addlinespace
Post-Covid $\times$ Low Hate Crime Rate&                     &                     &      0.0114\sym{***}&                     \\
                    &                     &                     &    (0.0024)         &                     \\
\addlinespace
Post-Covid $\times$ More Culturally Homogeneous&                     &                     &                     &      0.0106\sym{***}\\
                    &                     &                     &                     &    (0.0032)         \\
\midrule
Obs                 &     243,251         &     243,251         &     243,251         &     243,251         \\
Donor Fixed Effects &           Y         &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         \\
Total Donations     &           Y         &           Y         &           Y         &           Y         \\
Sectoral Composition Controls&           Y         &           Y         &           Y         &           Y         \\
Differential Effects by Other Socio-Economic Variables&           Y         &           Y         &           Y         &           Y         \\


==> results_table/heterogeneities_wocontrols2.tex <==
                    &\multicolumn{4}{c}{Local Share (Value)}                                                \\\cmidrule(lr){2-5}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\midrule
Post-Covid          &     -0.0096         &     -0.0074         &     -0.0078         &     -0.0080         \\
                    &    (0.0099)         &    (0.0097)         &    (0.0097)         &    (0.0098)         \\
\addlinespace
Post-Covid $\times$ High Covid&      0.0039         &      0.0035         &      0.0032         &      0.0034         \\
                    &    (0.0030)         &    (0.0030)         &    (0.0029)         &    (0.0031)         \\
\addlinespace
Post-Covid $\times$ Stronger Sense of Local Belonging&      0.0048\sym{**} &                     &                     &                     \\
                    &    (0.0022)         &                     &                     &                     \\
\addlinespace
Post-Covid $\times$ High Neighbourhood Cohesion&                     &      0.0012         &                     &                     \\
                    &                     &    (0.0027)         &                     &                     \\
\addlinespace
Post-Covid $\times$ Low Hate Crime Rate&                     &                     &      0.0026         &                     \\
                    &                     &                     &    (0.0026)         &                     \\
\addlinespace
Post-Covid $\times$ More Culturally Homogeneous&                     &                     &                     &      0.0010         \\
                    &                     &                     &                     &    (0.0028)         \\
\midrule
Obs                 &     276,090         &     276,090         &     276,090         &     276,090         \\
Donor Fixed Effects &           Y         &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         \\
Total Donations     &           Y         &           Y         &           Y         &           Y         \\
Sectoral Composition Controls&           Y         &           Y         &           Y         &           Y         \\
Differential Effects by Other Socio-Economic Variables&           Y         &           Y         &           Y         &           Y         \\


==> results_table/heterogeneities_wocontrols3.tex <==
                    &\multicolumn{4}{c}{Local Share (Value)}                                                \\\cmidrule(lr){2-5}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\midrule
Post-Covid          &     -0.0096         &     -0.0074         &     -0.0078         &     -0.0080         \\
                    &    (0.0099)         &    (0.0097)         &    (0.0097)         &    (0.0098)         \\
\addlinespace
Post-Covid $\times$ High Covid&      0.0039         &      0.0035         &      0.0032         &      0.0034         \\
                    &    (0.0030)         &    (0.0030)         &    (0.0029)         &    (0.0031)         \\
\addlinespace
Post-Covid $\times$ Stronger Sense of Local Belonging&      0.0048\sym{**} &                     &                     &                     \\
                    &    (0.0022)         &                     &                     &                     \\
\addlinespace
Post-Covid $\times$ High Neighbourhood Cohesion&                     &      0.0012         &                     &                     \\
                    &                     &    (0.0027)         &                     &                     \\
\addlinespace
Post-Covid $\times$ Low Hate Crime Rate&                     &                     &      0.0026         &                     \\
                    &                     &                     &    (0.0026)         &                     \\
\addlinespace
Post-Covid $\times$ More Culturally Homogeneous&                     &                     &                     &      0.0010         \\
                    &                     &                     &                     &    (0.0028)         \\
\midrule
Obs                 &     276,090         &     276,090         &     276,090         &     276,090         \\
Donor Fixed Effects &           Y         &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         \\
Total Donations     &           Y         &           Y         &           Y         &           Y         \\
Sectoral Composition Controls&           Y         &           Y         &           Y         &           Y         \\
Differential Effects by Other Socio-Economic Variables&           Y         &           Y         &           Y         &           Y         \\


==> results_table/local_on_wellbeing.tex <==
                    &\multicolumn{2}{c}{Yesterday Anxiety}      &\multicolumn{2}{c}{Yesterday Happiness}    &\multicolumn{2}{c}{Life Satisfaction}      &\multicolumn{2}{c}{Life Worthwhile}        \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         &\multicolumn{1}{c}{(7)}         &\multicolumn{1}{c}{(8)}         \\
\midrule
Post (2021–2022)    &      -0.058         &      -0.064         &       0.097\sym{***}&       0.099\sym{**} &       0.069\sym{*}  &       0.055         &       0.045         &       0.040         \\
                    &     (0.042)         &     (0.059)         &     (0.037)         &     (0.048)         &     (0.037)         &     (0.048)         &     (0.037)         &     (0.047)         \\
\addlinespace
Post (2021–2022) × High COVID&      -0.053         &      -0.052         &      -0.041         &      -0.041         &      -0.031         &      -0.028         &      -0.015         &      -0.014         \\
                    &     (0.057)         &     (0.058)         &     (0.048)         &     (0.048)         &     (0.046)         &     (0.046)         &     (0.047)         &     (0.047)         \\
\addlinespace
Post (2021–2022) × High Local Giving Rise&      -0.004         &       0.061         &      -0.068         &      -0.066         &      -0.068         &      -0.099         &      -0.063         &      -0.064         \\
                    &     (0.061)         &     (0.082)         &     (0.050)         &     (0.067)         &     (0.047)         &     (0.060)         &     (0.048)         &     (0.065)         \\
\addlinespace
Post (2021–2022) × High COVID × High Local Giving Rise&       0.019         &       0.008         &       0.131\sym{**} &       0.131\sym{*}  &       0.110\sym{*}  &       0.116\sym{*}  &       0.081         &       0.081         \\
                    &     (0.082)         &     (0.083)         &     (0.067)         &     (0.067)         &     (0.061)         &     (0.061)         &     (0.064)         &     (0.065)         \\
\midrule
Obs.                &      12,155         &      12,155         &      12,272         &      12,272         &      12,163         &      12,163         &      11,965         &      11,965         \\
Individual Fixed Effects&           Y         &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Post (2021–2022) × Strong Local Belonging&           N         &           Y         &           N         &           Y         &           N         &           Y         &           N         &           Y         \\
Post (2021–2022) × High COVID × Strong Local Belonging&           N         &           Y         &           N         &           Y         &           N         &           Y         &           N         &           Y         \\


==> results_table/main_diff_change_after_covid.tex <==
                    &\multicolumn{6}{c}{Share of Local Donations}                                                                                       \\\cmidrule(lr){2-7}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\midrule
Post Covid          &      0.0042\sym{***}&     -0.0061         &     -0.0018         &     -0.0031         &                     &                     \\
                    &    (0.0013)         &    (0.0143)         &    (0.0136)         &    (0.0133)         &                     &                     \\
\addlinespace
Post Covid $\times$ High Covid&                     &      0.0065\sym{**} &      0.0072\sym{***}&      0.0077\sym{***}&      0.0086\sym{***}&                     \\
                    &                     &    (0.0025)         &    (0.0023)         &    (0.0023)         &    (0.0022)         &                     \\
\addlinespace
Post Covid $\times$ Large GDP Shock&                     &                     &     -0.0069\sym{***}&     -0.0073\sym{***}&     -0.0039         &                     \\
                    &                     &                     &    (0.0022)         &    (0.0021)         &    (0.0024)         &                     \\
\addlinespace
Post Covid $\times$ Strong Local Belonging&                     &                     &                     &      0.0070\sym{***}&      0.0065\sym{***}&                     \\
                    &                     &                     &                     &    (0.0023)         &    (0.0023)         &                     \\
\addlinespace
Year = 2020         &                     &                     &                     &                     &                     &     -0.0013         \\
                    &                     &                     &                     &                     &                     &    (0.0141)         \\
\addlinespace
Year = 2021         &                     &                     &                     &                     &                     &     -0.0155         \\
                    &                     &                     &                     &                     &                     &    (0.0146)         \\
\addlinespace
Year = 2020 $\times$ High Covid&                     &                     &                     &                     &                     &      0.0093\sym{***}\\
                    &                     &                     &                     &                     &                     &    (0.0028)         \\
\addlinespace
Year = 2021 $\times$ High Covid&                     &                     &                     &                     &                     &      0.0035         \\
                    &                     &                     &                     &                     &                     &    (0.0032)         \\
\midrule
Obs.                &     251,037         &     243,245         &     243,245         &     243,245         &     243,245         &     243,245         \\
Donor Fixed Effects &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         &           N         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Differential Change by Other Demographic Features&           N         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Region by Year Fixed Effects&           N         &           N         &           N         &           N         &           Y         &           N         \\


==> results_table/main_diff_change_after_covid_contT.tex <==
                    &\multicolumn{5}{c}{Share of Local Donations}                                                                 \\\cmidrule(lr){2-6}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         \\
\midrule
Post Covid          &     -0.0116         &     -0.0084         &     -0.0102         &                     &                     \\
                    &    (0.0153)         &    (0.0142)         &    (0.0141)         &                     &                     \\
\addlinespace
Post Covid $\times$ Covid Death Rate&      1.1281         &      2.4615         &      2.8813         &      2.3654         &                     \\
                    &    (2.0263)         &    (2.0049)         &    (1.9641)         &    (2.3427)         &                     \\
\addlinespace
Post Covid $\times$ Large GDP Shock&                     &     -0.0069\sym{***}&     -0.0073\sym{***}&     -0.0044\sym{*}  &                     \\
                    &                     &    (0.0025)         &    (0.0024)         &    (0.0026)         &                     \\
\addlinespace
Post Covid $\times$ Strong Local Belonging&                     &                     &      0.0068\sym{***}&      0.0063\sym{***}&                     \\
                    &                     &                     &    (0.0023)         &    (0.0022)         &                     \\
\addlinespace
Year = 2020         &                     &                     &                     &                     &     -0.0115         \\
                    &                     &                     &                     &                     &    (0.0155)         \\
\addlinespace
Year = 2021         &                     &                     &                     &                     &     -0.0155         \\
                    &                     &                     &                     &                     &    (0.0160)         \\
\addlinespace
Year = 2020 $\times$ Covid Death Rate&                     &                     &                     &                     &      3.0470         \\
                    &                     &                     &                     &                     &    (2.2924)         \\
\addlinespace
Year = 2021 $\times$ Covid Death Rate&                     &                     &                     &                     &     -0.9595         \\
                    &                     &                     &                     &                     &    (2.3458)         \\
\midrule
Obs.                &     243,245         &     243,245         &     243,245         &     243,245         &     243,245         \\
Donor Fixed Effects &           Y         &           Y         &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         &           Y         &           Y         \\
Differential Change by Other Demographic Features&           Y         &           Y         &           Y         &           Y         &           Y         \\
Region by Year Fixed Effects&           N         &           N         &           N         &           Y         &           N         \\


==> results_table/main_diff_change_after_covid_totD.tex <==
                    &\multicolumn{7}{c}{Log (Total Donations)}                                                                                                                \\\cmidrule(lr){2-8}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         &\multicolumn{1}{c}{(7)}         \\
\midrule
Post Covid          &      0.1797\sym{***}&      1.5533\sym{***}&      1.5489\sym{***}&      1.5482\sym{***}&                     &                     &                     \\
                    &    (0.0171)         &    (0.2269)         &    (0.2250)         &    (0.2251)         &                     &                     &                     \\
\addlinespace
Post Covid $\times$ High Covid&                     &     -0.0724\sym{**} &     -0.0732\sym{**} &     -0.0729\sym{**} &     -0.1215\sym{**} &     -0.0321\sym{***}&                     \\
                    &                     &    (0.0337)         &    (0.0331)         &    (0.0329)         &    (0.0493)         &    (0.0082)         &                     \\
\addlinespace
Post Covid $\times$ Large GDP Shock&                     &                     &      0.0077         &      0.0075         &     -0.0228         &      0.0055         &                     \\
                    &                     &                     &    (0.0354)         &    (0.0357)         &    (0.0393)         &    (0.0096)         &                     \\
\addlinespace
Post Covid $\times$ Strong Local Belonging&                     &                     &                     &      0.0042         &      0.0106         &      0.0067         &                     \\
                    &                     &                     &                     &    (0.0359)         &    (0.0363)         &    (0.0109)         &                     \\
\addlinespace
Year = 2020         &                     &                     &                     &                     &                     &                     &     -0.0013         \\
                    &                     &                     &                     &                     &                     &                     &    (0.0141)         \\
\addlinespace
Year = 2021         &                     &                     &                     &                     &                     &                     &     -0.0155         \\
                    &                     &                     &                     &                     &                     &                     &    (0.0146)         \\
\addlinespace
Year = 2020 $\times$ High Covid&                     &                     &                     &                     &                     &                     &      0.0093\sym{***}\\
                    &                     &                     &                     &                     &                     &                     &    (0.0028)         \\
\addlinespace
Year = 2021 $\times$ High Covid&                     &                     &                     &                     &                     &                     &      0.0035         \\
                    &                     &                     &                     &                     &                     &                     &    (0.0032)         \\
\midrule
Obs.                &     423,409         &     410,599         &     410,599         &     410,599         &     410,599         &     243,245         &     243,245         \\
Donor Fixed Effects &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Differential Change by Other Demographic Features&           N         &           Y         &           Y         &           Y         &           Y         &           Y         &           Y         \\
Region by Year Fixed Effects&           N         &           N         &           N         &           N         &           Y         &           Y         &           N         \\
Include Only Non-zero Observations&           N         &           N         &           N         &           N         &           N         &           Y         &           N         \\


==> results_table/media_on_local_share.tex <==
                    &\multicolumn{1}{c}{Any Local Donation}&\multicolumn{1}{c}{Local Share (Value)}&\multicolumn{1}{c}{Local Share (Number)}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
High Covid $\times$ High Media $\times$ Post&      0.0112\sym{*}  &      0.0072\sym{**} &      0.0056\sym{**} \\
                    &    (0.0063)         &    (0.0028)         &    (0.0027)         \\
\addlinespace
High Covid $\times$ Low Media $\times$ Post&      0.0152         &      0.0044         &      0.0033         \\
                    &    (0.0095)         &    (0.0060)         &    (0.0046)         \\
\addlinespace
Low Covid $\times$ High Media $\times$ Post&      0.0120\sym{***}&      0.0054\sym{***}&      0.0049\sym{***}\\
                    &    (0.0036)         &    (0.0018)         &    (0.0018)         \\
\addlinespace
Low Covid $\times$ Low Media $\times$ Post&     -0.0123\sym{*}  &     -0.0026         &     -0.0005         \\
                    &    (0.0064)         &    (0.0025)         &    (0.0025)         \\
\midrule
Obs                 &     251,043         &     251,043         &     251,043         \\
Mean Outcome        &       0.470         &       0.173         &       0.160         \\
Donor FE            &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         \\


==> results_table/other_on_local_giving.tex <==
                    &\multicolumn{3}{c}{Local Share (Value)}                          \\\cmidrule(lr){2-4}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Post-Covid          &     -0.0108         &     -0.0089         &     -0.0107         \\
                    &    (0.0089)         &    (0.0087)         &    (0.0088)         \\
\addlinespace
Post Covid $\times$ High Covid&      0.0089\sym{***}&      0.0071\sym{***}&      0.0069\sym{***}\\
                    &    (0.0024)         &    (0.0024)         &    (0.0025)         \\
\addlinespace
Post Covid $\times$ Big GDP Shock&     -0.0094\sym{***}&     -0.0085\sym{***}&     -0.0097\sym{***}\\
                    &    (0.0022)         &    (0.0022)         &    (0.0022)         \\
\addlinespace
Post Covid $\times$ Stronger Sense of Local Belonging&      0.0095\sym{***}&                     &                     \\
                    &    (0.0024)         &                     &                     \\
\addlinespace
Post Covid $\times$ Low Hate Crime Rate&                     &      0.0106\sym{***}&                     \\
                    &                     &    (0.0024)         &                     \\
\addlinespace
Post Covid $\times$ More Culturally Homogeneous&                     &                     &      0.0110\sym{***}\\
                    &                     &                     &    (0.0028)         \\
\midrule
Obs                 &     243,245         &     243,245         &     243,245         \\
Donor Fixed Effects &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         \\
Total Donations     &           Y         &           Y         &           Y         \\
Sectoral Composition Controls&           Y         &           Y         &           Y         \\
Differential Effects by Other Socio-Economic Variables&           Y         &           Y         &           Y         \\


==> results_table/parallel_trend_test.tex <==
                    &\multicolumn{4}{c}{Share of Local Donations}                                           \\\cmidrule(lr){2-5}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\midrule
Fake Post (2015-2019)&      0.0203         &      0.0179         &      0.0178         &                     \\
                    &    (0.0249)         &    (0.0254)         &    (0.0254)         &                     \\
\addlinespace
Fake Post $\times$ High Covid&      0.0001         &     -0.0003         &     -0.0003         &      0.0008         \\
                    &    (0.0044)         &    (0.0042)         &    (0.0042)         &    (0.0044)         \\
\addlinespace
Fake Post $\times$ Large GDP Shock&                     &      0.0035         &      0.0034         &      0.0017         \\
                    &                     &    (0.0039)         &    (0.0040)         &    (0.0045)         \\
\addlinespace
Fake Post $\times$ Strong Local Belonging&                     &                     &      0.0005         &      0.0017         \\
                    &                     &                     &    (0.0040)         &    (0.0039)         \\
\midrule
Obs.                &     201,159         &     201,159         &     201,159         &     201,159         \\
Donor Fixed Effects &           Y         &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         &           Y         \\
Differential Change by Other Demographic Features&           Y         &           Y         &           Y         &           Y         \\
Region by Year Fixed Effects&           N         &           N         &           N         &           Y         \\


==> results_table/robustness_check_covariants.tex <==
                    &\multicolumn{3}{c}{Local Share (Value)}                          \\\cmidrule(lr){2-4}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Post Covid          &     -0.0031         &     -0.0031         &     -0.0061         \\
                    &    (0.0133)         &    (0.0136)         &    (0.0138)         \\
\addlinespace
Post Covid $\times$ High Covid&      0.0077\sym{***}&      0.0066\sym{***}&      0.0066\sym{***}\\
                    &    (0.0023)         &    (0.0023)         &    (0.0024)         \\
\addlinespace
Post Covid $\times$ Big GDP Shock&     -0.0073\sym{***}&     -0.0067\sym{***}&     -0.0075\sym{***}\\
                    &    (0.0021)         &    (0.0021)         &    (0.0022)         \\
\addlinespace
Post Covid $\times$ Strong Local Belonging&      0.0070\sym{***}&                     &                     \\
                    &    (0.0023)         &                     &                     \\
\addlinespace
Post Covid $\times$ Low Hate Crime Rate&                     &      0.0064\sym{***}&                     \\
                    &                     &    (0.0021)         &                     \\
\addlinespace
Post Covid $\times$ More Culturally Homogeneous&                     &                     &      0.0053\sym{**} \\
                    &                     &                     &    (0.0024)         \\
\midrule
Obs                 &     243,245         &     243,245         &     243,245         \\
Donor Fixed Effects &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         \\
Total Donations     &           Y         &           Y         &           Y         \\
Sectoral Composition Controls&           Y         &           Y         &           Y         \\
Differential Effects by Other Socio-Economic Variables&           Y         &           Y         &           Y         \\


==> results_table/robustness_check_covariates.tex <==
                    &\multicolumn{3}{c}{Local Share (Value)}                          \\\cmidrule(lr){2-4}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Post-Covid          &     -0.0048         &     -0.0048         &     -0.0092         \\
                    &    (0.0133)         &    (0.0137)         &    (0.0138)         \\
\addlinespace
Post Covid $\times$ High Covid&      0.0085\sym{***}&      0.0072\sym{***}&      0.0070\sym{***}\\
                    &    (0.0023)         &    (0.0023)         &    (0.0024)         \\
\addlinespace
Post Covid $\times$ Big GDP Shock&     -0.0079\sym{***}&     -0.0073\sym{***}&     -0.0082\sym{***}\\
                    &    (0.0021)         &    (0.0021)         &    (0.0022)         \\
\addlinespace
Post Covid $\times$ Stronger Sense of Local Belonging&      0.0073\sym{***}&                     &                     \\
                    &    (0.0023)         &                     &                     \\
\addlinespace
Post Covid $\times$ Low Hate Crime Rate&                     &      0.0078\sym{***}&                     \\
                    &                     &    (0.0022)         &                     \\
\addlinespace
Post Covid $\times$ More Culturally Homogeneous&                     &                     &      0.0074\sym{***}\\
                    &                     &                     &    (0.0025)         \\
\midrule
Obs                 &     243,245         &     243,245         &     243,245         \\
Donor Fixed Effects &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         \\
Total Donations     &           Y         &           Y         &           Y         \\
Sectoral Composition Controls&           Y         &           Y         &           Y         \\
Differential Effects by Other Socio-Economic Variables&           Y         &           Y         &           Y         \\


==> results_table/robustness_distance_thresholds.tex <==
                    &\multicolumn{3}{c}{Share of Local Donations}                     \\\cmidrule(lr){2-4}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Post Covid          &     -0.0087         &     -0.0031         &     -0.0040         \\
                    &    (0.0133)         &    (0.0133)         &    (0.0141)         \\
\addlinespace
Post Covid $\times$ High Covid&      0.0060\sym{***}&      0.0077\sym{***}&      0.0070\sym{***}\\
                    &    (0.0021)         &    (0.0023)         &    (0.0024)         \\
\addlinespace
Post Covid $\times$ Large GDP Shock&     -0.0059\sym{***}&     -0.0073\sym{***}&     -0.0050\sym{**} \\
                    &    (0.0020)         &    (0.0021)         &    (0.0022)         \\
\addlinespace
Post Covid $\times$ Strong Local Belonging&      0.0068\sym{***}&      0.0070\sym{***}&      0.0065\sym{***}\\
                    &    (0.0022)         &    (0.0023)         &    (0.0024)         \\
\midrule
Obs.                &     243,245         &     243,245         &     243,245         \\
Donor Fixed Effects &           Y         &           Y         &           Y         \\
Year Trend          &           Y         &           Y         &           Y         \\
Total Donation      &           Y         &           Y         &           Y         \\
Sectoral Composition&           Y         &           Y         &           Y         \\
Differential Change by Other Demographic Features&           Y         &           Y         &           Y         \\
Donations to Local Charities within a given distance&       10 km         &       25 km         &       50 km         \\


==> results_table/summary_statistics_caf_donation.tex <==
                    &        Mean&          sd&          p1&         p25&         p50&         p75&         p99&           N\\
\midrule
\textbf{Donor Level}&            &            &            &            &            &            &            &            \\
Number of years donated&        4.72&        2.76&        1.00&        2.00&        5.00&        8.00&        8.00&      64,417\\
\addlinespace \textbf{Donor Year Level}&            &            &            &            &            &            &            &            \\
Number of charities supported&        7.01&        8.08&        0.00&        2.00&        5.00&        9.00&       38.00&     304,059\\
Number of donations &       17.06&       27.61&        1.00&        3.00&        8.00&       19.00&      134.00&     304,059\\
Total donation amount&     2204.86&    30112.79&       20.00&      225.00&      590.00&     1580.00&    22982.00&     304,059\\
Any local donation  &        0.46&        0.50&        0.00&        0.00&        0.00&        1.00&        1.00&     304,059\\
Total local donation amount&      426.78&     5050.43&        0.00&        0.00&        0.00&      150.00&     6215.00&     304,059\\
Share of local donation&        0.17&        0.28&        0.00&        0.00&        0.00&        0.21&        1.00&     304,059\\


==> results_table/treatment_correlation.tex <==
                    &\multicolumn{1}{c}{High Covid Exposure}\\
\midrule
Big GDP Shock       &      0.0474         \\
                    &    (0.0924)         \\
\addlinespace
High Media Coverage &      0.1392         \\
                    &    (0.0868)         \\
\addlinespace
Has someone you personally know died of coronavirus?&      1.2792\sym{***}\\
                    &    (0.3470)         \\
\addlinespace
Worry about you, or someone you are close to, catching coronavirus&      2.1456\sym{***}\\
                    &    (0.5377)         \\
\addlinespace
Has your household monthly income decreased since the coronavirus outbreak?&     -0.9513\sym{***}\\
                    &    (0.3137)         \\
\addlinespace
Worry about the impact of coronavirus on the economy&     -2.9517\sym{***}\\
                    &    (0.7028)         \\
\addlinespace
Worry about the impact of coronavirus on your way of life&      0.8193         \\
                    &    (0.6483)         \\
\addlinespace
Constant            &      0.8071         \\
                    &    (0.5631)         \\
\midrule
Obs                 &         516         \\
RSquare             &       0.140         \\

